Learning to play the Chess Variant Crazyhouse above World Champion Level with Deep Neural Networks and Human Data

Deep neural networks have been successfully applied in learning the board games Go, chess and shogi without prior knowledge by making use of reinforcement learning. Although starting from zero knowledge has been shown to yield impressive results, it is associated with high computationally costs especially for complex games. With this paper, we present CrazyAra which is a neural network based engine solely trained in supervised manner for the chess variant crazyhouse. Crazyhouse is a game with a higher branching factor than chess and there is only limited data of lower quality available compared to AlphaGo. Therefore, we focus on improving efficiency in multiple aspects while relying on low computational resources. These improvements include modifications in the neural network design and training configuration, the introduction of a data normalization step and a more sample efficient Monte-Carlo tree search which has a lower chance to blunder. After training on 569,537 human games for 1.5 days we achieve a move prediction accuracy of 60.4%. During development, versions of CrazyAra played professional human players. Most notably, CrazyAra achieved a four to one win over 2017 crazyhouse world champion Justin Tan (aka LM Jann Lee) who is more than 400 Elo higher rated compared to the average player in our training set. Furthermore, we test the playing strength of CrazyAra on CPU against all participants of the second Crazyhouse Computer Championships 2017, winning against twelve of the thirteen participants. Finally, for CrazyAraFish we continue training our model on generated engine games. In ten long-time control matches playing Stockfish 10, CrazyAraFish wins three games and draws one out of ten matches.

==> figures/tikz/dataset/elo_rating.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.447058823529412,0.698039215686274}
\definecolor{color1}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}

\begin{axis}[
axis line style={white!80.0!black},
tick align=outside,
tick pos=left,
x grid style={white!80.0!black},
xlabel={Rating},
xmajorgrids,
xmin=1944.2, xmax=3171.8,
y grid style={white!80.0!black},
ylabel={Number of Players},
ymajorgrids,
ymin=0, ymax=143640
]
\draw[fill=color0,draw opacity=0] (axis cs:2000,0) rectangle (axis cs:2055.8,136800);
\draw[fill=color0,draw opacity=0] (axis cs:2055.8,0) rectangle (axis cs:2111.6,133987);
\draw[fill=color0,draw opacity=0] (axis cs:2111.6,0) rectangle (axis cs:2167.4,125838);
\draw[fill=color0,draw opacity=0] (axis cs:2167.4,0) rectangle (axis cs:2223.2,118612);
\draw[fill=color0,draw opacity=0] (axis cs:2223.2,0) rectangle (axis cs:2279,112473);
\draw[fill=color0,draw opacity=0] (axis cs:2279,0) rectangle (axis cs:2334.8,106459);
\draw[fill=color0,draw opacity=0] (axis cs:2334.8,0) rectangle (axis cs:2390.6,95739);
\draw[fill=color0,draw opacity=0] (axis cs:2390.6,0) rectangle (axis cs:2446.4,84684);
\draw[fill=color0,draw opacity=0] (axis cs:2446.4,0) rectangle (axis cs:2502.2,65648);
\draw[fill=color0,draw opacity=0] (axis cs:2502.2,0) rectangle (axis cs:2558,46862);
\draw[fill=color0,draw opacity=0] (axis cs:2558,0) rectangle (axis cs:2613.8,34633);
\draw[fill=color0,draw opacity=0] (axis cs:2613.8,0) rectangle (axis cs:2669.6,25744);
\draw[fill=color0,draw opacity=0] (axis cs:2669.6,0) rectangle (axis cs:2725.4,19196);
\draw[fill=color0,draw opacity=0] (axis cs:2725.4,0) rectangle (axis cs:2781.2,14622);
\draw[fill=color0,draw opacity=0] (axis cs:2781.2,0) rectangle (axis cs:2837,8478);
\draw[fill=color0,draw opacity=0] (axis cs:2837,0) rectangle (axis cs:2892.8,5016);
\draw[fill=color0,draw opacity=0] (axis cs:2892.8,0) rectangle (axis cs:2948.6,2593);
\draw[fill=color0,draw opacity=0] (axis cs:2948.6,0) rectangle (axis cs:3004.4,979);
\draw[fill=color0,draw opacity=0] (axis cs:3004.4,0) rectangle (axis cs:3060.2,520);
\draw[fill=color0,draw opacity=0] (axis cs:3060.2,0) rectangle (axis cs:3116,189);
\addplot [thick, color1, forget plot]
table [row sep=\\]{%
2279.61423948618	0 \\
2279.61423948618	1 \\
};
\node at (axis cs:2325.2065242759,125000)[
  scale=0.6,
  anchor=base west,
  text=white!15.0!black,
  rotate=0.0
]{ mean=2279.61};
\end{axis}

\end{tikzpicture}

==> figures/tikz/dataset/top_active_cz_players.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.205659361783929,0.242445213379469,0.256470588235294}
\definecolor{color1}{rgb}{0.211318723567859,0.284890426758939,0.312941176470588}
\definecolor{color2}{rgb}{0.216978085351788,0.327335640138408,0.369411764705882}
\definecolor{color3}{rgb}{0.222637447135717,0.369780853517878,0.425882352941176}
\definecolor{color4}{rgb}{0.228296808919646,0.412226066897347,0.482352941176471}
\definecolor{color5}{rgb}{0.23442778418557,0.458208381391772,0.543529411764706}
\definecolor{color6}{rgb}{0.240087145969499,0.500653594771242,0.6}
\definecolor{color7}{rgb}{0.245746507753428,0.543098808150711,0.656470588235294}
\definecolor{color8}{rgb}{0.251405869537357,0.585544021530181,0.712941176470588}
\definecolor{color9}{rgb}{0.257065231321287,0.62798923490965,0.769411764705882}
\definecolor{color10}{rgb}{0.282855312059464,0.662909137511214,0.796468025118544}
\definecolor{color11}{rgb}{0.32480840702294,0.684931436626938,0.789947456106626}
\definecolor{color12}{rgb}{0.366761501986415,0.706953735742663,0.783426887094707}
\definecolor{color13}{rgb}{0.408714596949891,0.728976034858388,0.776906318082789}
\definecolor{color14}{rgb}{0.450667691913367,0.750998333974113,0.77038574907087}
\definecolor{color15}{rgb}{0.496116878123799,0.774855824682814,0.763321799307959}
\definecolor{color16}{rgb}{0.538069973087274,0.796878123798539,0.75680123029604}
\definecolor{color17}{rgb}{0.58002306805075,0.818900422914264,0.750280661284122}
\definecolor{color18}{rgb}{0.621976163014225,0.840922722029988,0.743760092272203}
\definecolor{color19}{rgb}{0.663929257977701,0.862945021145713,0.737239523260285}

\begin{axis}[
axis line style={white!80.0!black},
tick align=outside,
tick pos=left,
x grid style={white!80.0!black},
xlabel={Number of Games},
xmajorgrids,
xmin=0, xmax=27048,
y grid style={white!80.0!black},
ylabel={Crazyhouse Players on lichess.org},
ymajorgrids,
ymin=-0.5, ymax=19.5,
ytick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19},
yticklabels={trataredeganart,Masalanka,JohnStuckey,HighContrast,Flourish,kayhiking,matser,emrty,mastertan,saturos,opperwezen,mariorton,crosky,JannLee,KyleLegion,dovijanic,xuanet,retardedplatypus123,ciw,mathace}
]
\addlegendimage{ybar,ybar legend,fill=color0,draw opacity=0};
\draw[fill=color0,draw opacity=0] (axis cs:0,-0.25) rectangle (axis cs:7657,0.25);
\draw[fill=color1,draw opacity=0] (axis cs:0,0.75) rectangle (axis cs:7730,1.25);
\draw[fill=color2,draw opacity=0] (axis cs:0,1.75) rectangle (axis cs:7870,2.25);
\draw[fill=color3,draw opacity=0] (axis cs:0,2.75) rectangle (axis cs:7939,3.25);
\draw[fill=color4,draw opacity=0] (axis cs:0,3.75) rectangle (axis cs:8025,4.25);
\draw[fill=color5,draw opacity=0] (axis cs:0,4.75) rectangle (axis cs:8051,5.25);
\draw[fill=color6,draw opacity=0] (axis cs:0,5.75) rectangle (axis cs:8165,6.25);
\draw[fill=color7,draw opacity=0] (axis cs:0,6.75) rectangle (axis cs:9075,7.25);
\draw[fill=color8,draw opacity=0] (axis cs:0,7.75) rectangle (axis cs:11925,8.25);
\draw[fill=color9,draw opacity=0] (axis cs:0,8.75) rectangle (axis cs:11999,9.25);
\draw[fill=color10,draw opacity=0] (axis cs:0,9.75) rectangle (axis cs:12902,10.25);
\draw[fill=color11,draw opacity=0] (axis cs:0,10.75) rectangle (axis cs:13438,11.25);
\draw[fill=color12,draw opacity=0] (axis cs:0,11.75) rectangle (axis cs:14308,12.25);
\draw[fill=color13,draw opacity=0] (axis cs:0,12.75) rectangle (axis cs:14359,13.25);
\draw[fill=color14,draw opacity=0] (axis cs:0,13.75) rectangle (axis cs:15203,14.25);
\draw[fill=color15,draw opacity=0] (axis cs:0,14.75) rectangle (axis cs:17896,15.25);
\draw[fill=color16,draw opacity=0] (axis cs:0,15.75) rectangle (axis cs:19269,16.25);
\draw[fill=color17,draw opacity=0] (axis cs:0,16.75) rectangle (axis cs:19634,17.25);
\draw[fill=color18,draw opacity=0] (axis cs:0,17.75) rectangle (axis cs:20933,18.25);
\draw[fill=color19,draw opacity=0] (axis cs:0,18.75) rectangle (axis cs:25760,19.25);
\path [draw=white!80.0!black, fill opacity=0] (axis cs:0,-0.5)
--(axis cs:0,19.5);

\path [draw=white!80.0!black, fill opacity=0] (axis cs:1,-0.5)
--(axis cs:1,19.5);

\path [draw=white!80.0!black, fill opacity=0] (axis cs:0,0)
--(axis cs:27048,0);

\path [draw=white!80.0!black, fill opacity=0] (axis cs:0,1)
--(axis cs:27048,1);

\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 20th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 19th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 18th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 17th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 16th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 15th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 14th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 13th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 12th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 11th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 10th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 9th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 8th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 7th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 6th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 5th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 4th};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 3rd};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 2nd};
\node at (axis cs:5,0)[
  scale=0.5,
  anchor= west,
  text=black,
  rotate=0.0
]{ 1st};
\end{axis}

\end{tikzpicture}

==> figures/tikz/elo_increase/relative_elo_increase.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.447058823529412,0.698039215686274}
\definecolor{color1}{rgb}{0,0.619607843137255,0.450980392156863}
\definecolor{color2}{rgb}{0.835294117647059,0.368627450980392,0}

\begin{axis}[
axis line style={white!80.0!black},
legend cell align={left},
legend entries={{default},{with-q-values},{with-q-pv-values}},
legend style={at={(0.97,0.03)}, anchor=south east, draw=none},
tick align=outside,
tick pos=left,
x grid style={white!80.0!black},
xlabel={Number of Simulations per Move},
xmajorgrids,
xmin=720, xmax=2480,
y grid style={white!80.0!black},
ylabel={Relative Elo},
ymajorgrids,
ymin=-92.653, ymax=666.633
]
\addlegendimage{no markers, color0}
\addlegendimage{no markers, color1}
\addlegendimage{no markers, color2}
\path [fill=color0, fill opacity=0.05] (axis cs:800,0)
--(axis cs:800,0)
--(axis cs:1600,151.94)
--(axis cs:2400,294.2)
--(axis cs:2400,632.12)
--(axis cs:2400,632.12)
--(axis cs:1600,329.7)
--(axis cs:800,0)
--cycle;

\path [fill=color1, fill opacity=0.05] (axis cs:800,79)
--(axis cs:800,-58.14)
--(axis cs:1600,227.12)
--(axis cs:2400,273.46)
--(axis cs:2400,571.3)
--(axis cs:2400,571.3)
--(axis cs:1600,448.96)
--(axis cs:800,79)
--cycle;

\path [fill=color2, fill opacity=0.05] (axis cs:800,79)
--(axis cs:800,-13.07)
--(axis cs:1600,220.17)
--(axis cs:2400,253.38)
--(axis cs:2400,571.3)
--(axis cs:2400,571.3)
--(axis cs:1600,448.96)
--(axis cs:800,79)
--cycle;

\addplot [semithick, color0, opacity=0.25, dashed, forget plot]
table [row sep=\\]{%
800	0 \\
1600	151.94 \\
2400	294.2 \\
};
\addplot [semithick, color0, opacity=0.25, dashed, forget plot]
table [row sep=\\]{%
800	0 \\
1600	329.7 \\
2400	632.12 \\
};
\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table [row sep=\\]{%
800	0 \\
1600	240.82 \\
2400	463.16 \\
};
\addplot [semithick, color1, mark=*, mark size=3, mark options={solid}]
table [row sep=\\]{%
800	10.43 \\
1600	338.04 \\
2400	422.38 \\
};
\addplot [semithick, color1, opacity=0.25, dashed, forget plot]
table [row sep=\\]{%
800	-58.14 \\
1600	227.12 \\
2400	273.46 \\
};
\addplot [semithick, color1, opacity=0.25, dashed, forget plot]
table [row sep=\\]{%
800	79 \\
1600	448.96 \\
2400	571.3 \\
};
\addplot [semithick, color2, mark=*, mark size=3, mark options={solid}]
table [row sep=\\]{%
800	56.07 \\
1600	330.23 \\
2400	381.69 \\
};
\addplot [semithick, color2, opacity=0.25, dashed, forget plot]
table [row sep=\\]{%
800	-13.07 \\
1600	220.17 \\
2400	253.38 \\
};
\addplot [semithick, color2, opacity=0.25, dashed, forget plot]
table [row sep=\\]{%
800	125.21 \\
1600	440.29 \\
2400	510 \\
};
\end{axis}

\end{tikzpicture}

==> figures/tikz/elo_increase/relative_elo_increase_old.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
axis line style={white!80.0!black},
legend cell align={left},
legend entries={{default},{with-q-values}},
legend style={draw=none},
tick align=outside,
tick pos=left,
x grid style={white!80.0!black},
xlabel={Number of Simulations per Move},
xmajorgrids,
xmin=720, xmax=2480,
y grid style={white!80.0!black},
ylabel={Relative Elo},
ymajorgrids,
ymin=-92.653, ymax=666.633
]
\addlegendimage{no markers, color0}
\addlegendimage{no markers, color1}
\path [fill=color0, fill opacity=0.1] (axis cs:800,0)
--(axis cs:800,0)
--(axis cs:1600,151.94)
--(axis cs:2400,294.2)
--(axis cs:2400,632.12)
--(axis cs:2400,632.12)
--(axis cs:1600,329.7)
--(axis cs:800,0)
--cycle;

\path [fill=color1, fill opacity=0.1] (axis cs:800,79)
--(axis cs:800,-58.14)
--(axis cs:1600,227.12)
--(axis cs:2400,273.46)
--(axis cs:2400,571.3)
--(axis cs:2400,571.3)
--(axis cs:1600,448.96)
--(axis cs:800,79)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table [row sep=\\]{%
800	0 \\
1600	240.82 \\
2400	463.16 \\
};
\addplot [semithick, color1, mark=*, mark size=3, mark options={solid}]
table [row sep=\\]{%
800	10.43 \\
1600	338.04 \\
2400	422.38 \\
};
\end{axis}

\end{tikzpicture}

==> figures/tikz/mcts/q_values.tex <==
% This file was created by tikzplotlib v0.8.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.419607843137255,0.643137254901961}
\definecolor{color1}{rgb}{1,0.501960784313725,0.0549019607843137}
\definecolor{color2}{rgb}{0.372549019607843,0.619607843137255,0.819607843137255}

\begin{axis}[
axis line style={white!80.0!black},
legend cell align={left},
legend style={at={(0.97,0.03)}, anchor=south east, draw=white!80.0!black},
tick align=outside,
tick pos=both,
x grid style={white!80.0!black},
xlabel={Total Simulations},
xmin=-1620.85, xmax=34125.85,
xtick style={color=white!15.0!black},
xtick={-5000,0,5000,10000,15000,20000,25000,30000,35000},
xticklabels={\(\displaystyle -5000\),\(\displaystyle 0\),\(\displaystyle 5000\),\(\displaystyle 10000\),\(\displaystyle 15000\),\(\displaystyle 20000\),\(\displaystyle 25000\),\(\displaystyle 30000\),\(\displaystyle 35000\)},
y grid style={white!80.0!black},
ylabel={Q-Value for N@e6},
ymajorgrids,
ymin=-1.0901433, ymax=0.8930093,
ytick style={color=white!15.0!black},
ytick={-1.25,-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={\(\displaystyle -1.25\),\(\displaystyle -1.00\),\(\displaystyle -0.75\),\(\displaystyle -0.50\),\(\displaystyle -0.25\),\(\displaystyle 0.00\),\(\displaystyle 0.25\),\(\displaystyle 0.50\),\(\displaystyle 0.75\),\(\displaystyle 1.00\)}
]
\addplot [semithick, color0]
table {%
4 -1
231 -1
444 -1
626 -1
815 -1
1002 -1
1201 -1
1364 -1
1529 -1
1692 -1
1862 -1
2070 -1
2274 -1
2449 -1
2610 -1
2788 -1
2971 -1
3148 -1
3325 -1
3511 -1
3748 -1
3936 -1
4110 -1
4329 -1
4564 -1
4766 -1
5019 -1
5233 -1
5465 -1
5659 -1
5868 -1
6107 -1
6368 -1
6581 -1
6784 -1
6954 -1
7118 -1
7279 -1
7440 -1
7656 -1
7870 -1
8043 -1
8232 -1
8439 -1
8634 -1
8816 -1
9010 -1
9212 -1
9390 -1
9552 -1
9716 -1
9894 -1
10069 -1
10241 -1
10416 -1
10581 -1
10741 -1
10901 -1
11063 -1
11246 -1
11436 -1
11614 -1
11819 -1
11992 -1
12152 -1
12333 0.597334
12548 0.24798
12729 0.20501
12919 0.138578
13113 0.138578
13305 0.138578
13476 0.138578
13679 0.138578
13858 0.138578
14037 0.138578
14229 0.138578
14424 0.138578
14590 0.138578
14783 0.138578
14977 0.138578
15185 0.138578
15371 0.138578
15578 0.134878
15748 0.134878
15916 0.134878
16108 0.259089
16333 0.116609
16577 0.0845997
16783 0.0845997
17052 0.064938
17303 0.049439
17499 0.0395387
17688 0.0395387
17896 0.0395387
18138 0.0216041
18345 0.0216041
18552 0.0131228
18758 0.0131228
18995 0.00438009
19260 0.0113361
19510 -0.0183923
19710 -0.0183923
19960 -0.0326592
20224 -0.0438546
20476 -0.0578829
20682 -0.0578829
20869 -0.0568169
21103 -0.0703332
21328 -0.0625415
21558 -0.079061
21737 -0.079061
21914 -0.079061
22129 -0.0802954
22332 -0.086191
22578 -0.0885948
22786 0.0648572
22962 0.0585261
23129 0.000683882
23334 -0.044906
23549 -0.0527793
23788 0.127176
24031 0.220156
24225 0.206484
24391 0.268281
24558 0.292904
24740 0.253887
24920 0.210613
25096 0.168585
25268 0.166359
25428 0.201897
25590 0.236652
25752 0.265223
25915 0.277274
26081 0.297046
26243 0.292066
26406 0.277132
26571 0.281742
26745 0.302291
26916 0.316155
27086 0.328088
27248 0.329491
27423 0.340375
27604 0.354668
27788 0.368546
27968 0.382322
28145 0.387753
28334 0.398504
28522 0.401762
28714 0.413661
28887 0.418821
29062 0.423801
29224 0.419951
29396 0.428003
29574 0.43429
29744 0.436759
29913 0.444344
30092 0.453102
30275 0.461786
30453 0.46993
30635 0.477723
30814 0.484292
30995 0.487577
31189 0.496604
31380 0.504305
31575 0.510537
31760 0.51649
31931 0.517509
32116 0.522124
};
\addlegendentry{default}
\addplot [semithick, color1]
table {%
4 -1
232 -1
452 -1
635 -1
838 -1
1040 -1
1217 -1
1380 -1
1542 -1
1706 -1
1882 -1
2112 -1
2288 -1
2463 -1
2626 -1
2809 -1
2997 -1
3171 -1
3344 -1
3540 -1
3759 -1
3953 -1
4130 -1
4361 -1
4603 -1
4809 -1
5046 -1
5260 -1
5498 -1
5672 -1
5881 -1
6105 -1
6364 -1
6599 -1
6791 -1
6982 -1
7146 -1
7306 -1
7468 -1
7649 -1
7890 -1
8067 -1
8251 -1
8446 -1
8645 -1
8821 -1
9006 -1
9213 -1
9389 -1
9550 -1
9713 -1
9887 -1
10065 -1
10238 -1
10419 -1
10591 -1
10751 -1
10911 -1
11073 -1
11265 -1
11453 -1
11635 -1
11826 -1
11999 -1
12159 -1
12340 0.597334
12557 0.24798
12738 0.214796
12925 0.134878
13124 0.134878
13330 0.134878
13496 0.134878
13701 0.134878
13893 0.134878
14069 0.134878
14258 0.134878
14437 0.134878
14617 0.134878
14827 0.134878
15021 0.366249
15225 0.144235
15428 0.144235
15606 0.144235
15827 0.122776
15991 0.122776
16158 0.122776
16337 0.122776
16555 0.0992978
16808 0.0781275
17029 0.0670128
17248 0.0561249
17465 0.0471106
17653 0.0471106
17895 0.0418947
18137 0.0216638
18326 0.0216638
18549 0.0132069
18779 0.0035573
18990 0.0035573
19246 -0.0135384
19480 -0.0226723
19687 -0.0226723
19953 -0.0243039
20165 -0.0342771
20343 -0.0342771
20557 -0.0414186
20808 -0.0486308
21079 -0.059839
21334 -0.067071
21576 -0.079041
21738 -0.079041
21949 -0.0859138
22170 -0.0905297
22414 -0.102418
22659 -0.0710834
22836 0.0340068
23011 0.0652378
23187 0.00295185
23354 -0.0375996
23572 -0.0177694
23820 0.141734
24050 0.185209
24237 0.197772
24404 0.253869
24572 0.273853
24747 0.233981
24933 0.182484
25113 0.145013
25279 0.16666
25441 0.208083
25604 0.237681
25765 0.262832
25929 0.272865
26092 0.286567
26255 0.270779
26417 0.269113
26590 0.283071
26760 0.301333
26931 0.318162
27098 0.320411
27266 0.327674
27443 0.340882
27624 0.354264
27810 0.369157
27992 0.380305
28169 0.383342
28357 0.397035
28542 0.400728
28724 0.41009
28895 0.417128
29085 0.426668
29253 0.43131
29432 0.438475
29597 0.432111
29764 0.438778
29933 0.440742
30110 0.449497
30291 0.457774
30474 0.466694
30652 0.474534
30834 0.48021
31015 0.486934
31204 0.495769
31401 0.50321
31598 0.508253
31777 0.512955
31950 0.514169
32135 0.52007
32323 0.524822
32501 0.528951
};
\addlegendentry{fix-checkmates}
\addplot [semithick, white!67.05882352941175!black]
table {%
5 0.802866
216 0.238116
403 0.268416
603 0.0238427
782 -0.0210083
971 -0.0210083
1190 -0.0210083
1416 -0.0210083
1647 -0.0210083
1886 -0.0210083
2124 -0.0210083
2290 -0.0210083
2455 -0.0210083
2626 -0.0210083
2804 -0.0210083
2978 -0.0210083
3144 -0.0210083
3318 -0.0210083
3483 -0.0210083
3644 -0.0210083
3807 -0.0210083
3972 -0.0210083
4146 -0.0210083
4322 -0.0210083
4506 -0.0210083
4687 -0.0210083
4880 -0.0210083
5079 -0.0210083
5260 -0.0210083
5434 -0.0210083
5626 -0.0210083
5842 -0.0210083
6051 -0.0210083
6258 -0.0210083
6467 -0.0210083
6659 -0.0210083
6876 -0.0257526
7065 -0.0345643
7262 -0.0394779
7483 -0.0603682
7697 -0.0716138
7896 -0.0734426
8074 -0.0386306
8235 -0.0708863
8406 -0.0708863
8573 -0.0708863
8735 -0.0708863
8897 -0.0708863
9058 -0.0708863
9258 -0.0708863
9436 -0.0708863
9601 -0.0708863
9762 -0.0708863
9925 -0.0708863
10118 -0.0708863
10342 -0.0708863
10575 -0.0708863
10803 -0.0907397
11043 -0.0789637
11260 -0.102637
11479 -0.118461
11694 -0.115985
11923 -0.0849722
12151 0.101423
12400 0.252578
12579 0.275243
12764 0.260788
12924 0.295538
13085 0.33175
13273 0.375538
13479 0.413415
13679 0.442901
13889 0.476598
14088 0.498546
14307 0.523433
14497 0.532151
14675 0.540127
14876 0.553501
15077 0.559093
15237 0.548054
15399 0.55161
15568 0.561183
15735 0.548855
15902 0.535227
16064 0.519816
16228 0.497642
16392 0.492448
16564 0.498104
16732 0.506995
16903 0.513027
17067 0.508208
17228 0.503372
17396 0.50672
17561 0.502738
17724 0.498844
17889 0.502443
18060 0.50645
18228 0.511053
18394 0.50794
18562 0.501628
18733 0.498068
18910 0.503584
19090 0.509581
19261 0.516475
19441 0.521483
19617 0.525709
19786 0.528546
19954 0.533593
20129 0.539719
20308 0.544293
20494 0.54906
20682 0.555028
20867 0.555866
21040 0.557496
21226 0.562734
21407 0.565971
21586 0.570144
21779 0.576265
21983 0.581532
22175 0.585523
22363 0.588785
22555 0.593177
22747 0.597391
22942 0.601121
23123 0.602804
23318 0.605549
23493 0.606435
23682 0.609358
23869 0.613002
24058 0.615819
24257 0.619243
24451 0.622547
24653 0.625472
24854 0.628535
25043 0.626526
25235 0.625538
25409 0.624163
25593 0.623955
25787 0.623328
25970 0.625057
26158 0.626719
26348 0.626741
26530 0.626301
26700 0.624664
26869 0.62246
27040 0.62193
27211 0.619773
27380 0.61794
27550 0.616227
27720 0.613889
27883 0.610528
28054 0.610205
28221 0.607873
28386 0.604464
28558 0.602029
28721 0.599375
28893 0.596028
29060 0.595734
29234 0.595627
29410 0.593595
29582 0.593771
29747 0.593006
29918 0.593014
30095 0.592678
};
\addlegendentry{enhance-checks}
\addplot [semithick, white!34.90196078431372!black]
table {%
4 -1
227 -1
435 -1
609 -1
785 -1
977 -1
1140 -1
1300 -1
1463 -1
1633 -1
1798 -1
1970 -1
2138 -1
2307 -1
2479 -1
2652 -1
2855 -1
3049 -1
3217 -1
3401 -1
3572 -1
3741 -1
3920 0.507644
4086 0.507644
4257 0.507644
4440 0.461544
4645 0.391947
4854 0.307488
5041 0.307488
5242 0.295979
5432 0.24798
5650 0.24798
5833 0.24798
6030 0.24798
6243 0.203409
6469 0.203409
6653 0.214796
6844 0.214796
7022 0.214796
7210 0.214796
7434 0.20501
7635 0.178183
7802 0.178183
7968 0.178183
8130 0.178183
8300 0.178183
8513 0.178183
8747 0.149238
8941 0.149238
9185 0.138578
9400 0.134878
9595 0.334787
9783 0.200001
9969 0.150432
10201 0.125736
10454 0.102935
10704 0.0919248
10963 0.0698344
11229 0.0582057
11505 0.0403786
11746 0.0300804
11976 0.0204577
12233 0.00127825
12432 0.00127825
12627 0.00127825
12857 -0.00873453
13115 -0.0169282
13290 -0.0169282
13506 -0.0169282
13710 -0.0183093
13929 -0.019401
14167 -0.0300489
14433 -0.0453104
14661 -0.0532004
14853 -0.0532004
15032 -0.0532004
15231 -0.0532004
15464 -0.0606004
15686 -0.064881
15878 -0.064881
16108 -0.0724223
16359 -0.0782517
16618 -0.0869866
16859 -0.0942749
17087 -0.0967486
17295 0.0612652
17466 0.0530876
17640 -0.034926
17821 -0.0672448
17987 -0.0902972
18157 -0.0902972
18331 -0.0902972
18496 -0.0902972
18756 -0.0995559
18990 -0.105003
19165 -0.105003
19331 -0.105003
19505 -0.105003
19771 -0.104864
19994 0.0302691
20246 0.182992
20477 0.15476
20639 0.22608
20807 0.259099
20979 0.249625
21158 0.20361
21332 0.188279
21492 0.223821
21655 0.259665
21817 0.287702
21979 0.304898
22146 0.318265
22310 0.316175
22473 0.299889
22636 0.295525
22809 0.311426
22983 0.32582
23165 0.33812
23336 0.338663
23503 0.346153
23681 0.36174
23865 0.377026
24056 0.392869
24240 0.407826
24417 0.410179
24606 0.424545
24799 0.439192
24983 0.45115
25173 0.461267
25364 0.472818
25554 0.483515
25744 0.493282
25944 0.501254
26119 0.504571
26311 0.513152
26519 0.521792
26706 0.529126
26883 0.531186
27058 0.534174
27253 0.540247
27432 0.544143
27606 0.545253
27778 0.54298
27944 0.545041
28131 0.549786
28327 0.556549
28497 0.560541
28683 0.563995
28855 0.566217
29047 0.570876
29228 0.575011
29422 0.579826
29606 0.580104
29784 0.582276
29977 0.586044
30155 0.58855
30356 0.591955
30550 0.594974
30740 0.598873
30928 0.601608
31113 0.604305
31300 0.605538
31477 0.607019
31659 0.60969
31852 0.612182
32032 0.614907
32225 0.616963
32401 0.618955
};
\addlegendentry{u-value-exploration-factor}
\addplot [semithick, color2]
table {%
5 0.802866
216 0.238116
404 0.25587
593 0.0666394
771 0.0654624
948 0.0617353
1113 0.0617353
1273 0.0617353
1435 0.0617353
1596 0.0617353
1758 0.0617353
1923 0.0617353
2089 0.0617353
2252 0.0617353
2419 0.0617353
2592 0.0617353
2760 0.0617353
2930 0.0617353
3098 0.0617353
3268 0.0617353
3445 0.0617353
3635 0.0617353
3827 0.0617353
4012 0.0617353
4190 0.0617353
4366 0.0617353
4533 0.0617353
4697 0.0617353
4857 0.0617353
5019 0.0617353
5187 0.0617353
5349 0.0617353
5516 0.0617353
5682 0.0617353
5847 0.0617353
6019 0.0617353
6193 0.0617353
6365 0.0617353
6527 0.0617353
6694 0.0617353
6864 0.0617353
7037 0.0617353
7216 0.0617353
7386 0.0617353
7570 0.0617353
7740 0.0617353
7934 0.0617353
8161 0.0617353
8378 0.0617353
8550 0.0617353
8730 0.0617353
8920 0.0617353
9135 0.0617353
9377 0.0617353
9614 0.0617353
9842 0.0617353
10087 0.0390397
10337 0.0314972
10592 0.0147054
10827 0.0147054
11053 0.0147054
11297 0.0147054
11532 0.0147054
11758 0.0147054
11926 0.0147054
12094 0.0147054
12272 0.0147054
12467 0.0147054
12640 0.0147054
12833 0.0147054
13022 0.0147054
13228 0.00942043
13473 -0.0144625
13709 -0.0233093
13882 -0.0233093
14048 -0.0233093
14214 -0.0233093
14473 -0.0332077
14734 -0.0444935
14986 -0.0555098
15236 -0.0625216
15422 -0.0662428
15582 -0.0662428
15756 -0.0700129
16010 -0.0790562
16262 -0.077069
16521 -0.0789666
16726 -0.0543836
16948 -0.0700752
17180 -0.0805417
17403 -0.0865697
17651 -0.0557146
17878 -0.094114
18131 -0.103616
18390 -0.114967
18638 -0.117208
18885 -0.127063
19098 -0.131216
19330 -0.00288377
19576 0.1822
19808 0.27743
19985 0.257815
20155 0.277919
20316 0.316737
20479 0.351619
20688 0.399732
20886 0.429733
21095 0.458551
21310 0.484791
21513 0.511813
21704 0.524527
21887 0.529108
22061 0.532279
22224 0.538959
22429 0.555332
22632 0.569238
22821 0.575905
23003 0.579131
23207 0.590073
23388 0.589316
23550 0.574892
23716 0.561821
23879 0.546688
24041 0.530966
24205 0.518805
24371 0.513527
24537 0.51482
24706 0.518128
24876 0.523353
25046 0.527787
25208 0.526412
25377 0.530353
25545 0.536813
25714 0.543297
25887 0.547781
26057 0.551447
26228 0.557681
26400 0.564294
26575 0.571057
26747 0.574113
26917 0.578843
27086 0.582156
27252 0.579407
27431 0.582101
27625 0.587132
27811 0.592624
28011 0.597696
28210 0.603417
28388 0.605211
28572 0.608798
28752 0.610982
28951 0.614217
29132 0.613652
29321 0.616852
29504 0.619876
29686 0.621876
29874 0.626236
30062 0.626559
30239 0.626598
30430 0.624709
};
\addlegendentry{all}
\end{axis}

\end{tikzpicture}

==> figures/tikz/mcts/simulations.tex <==
% This file was created by tikzplotlib v0.8.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.419607843137255,0.643137254901961}
\definecolor{color1}{rgb}{1,0.501960784313725,0.0549019607843137}
\definecolor{color2}{rgb}{0.372549019607843,0.619607843137255,0.819607843137255}

\begin{axis}[
axis line style={white!80.0!black},
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black},
tick align=outside,
tick pos=both,
x grid style={white!80.0!black},
xlabel={Total Simulations},
xmin=-1620.85, xmax=34125.85,
xtick style={color=white!15.0!black},
xtick={-5000,0,5000,10000,15000,20000,25000,30000,35000},
xticklabels={\(\displaystyle -5000\),\(\displaystyle 0\),\(\displaystyle 5000\),\(\displaystyle 10000\),\(\displaystyle 15000\),\(\displaystyle 20000\),\(\displaystyle 25000\),\(\displaystyle 30000\),\(\displaystyle 35000\)},
y grid style={white!80.0!black},
ylabel={Simulations for N@e6},
ymajorgrids,
ymin=-941.5, ymax=19771.5,
ytick style={color=white!15.0!black},
ytick={-2500,0,2500,5000,7500,10000,12500,15000,17500,20000},
yticklabels={\(\displaystyle -2500\),\(\displaystyle 0\),\(\displaystyle 2500\),\(\displaystyle 5000\),\(\displaystyle 7500\),\(\displaystyle 10000\),\(\displaystyle 12500\),\(\displaystyle 15000\),\(\displaystyle 17500\),\(\displaystyle 20000\)}
]
\addplot [semithick, color0]
table {%
4 0
231 0
444 0
626 0
815 0
1002 0
1201 0
1364 0
1529 0
1692 0
1862 0
2070 0
2274 0
2449 0
2610 0
2788 0
2971 0
3148 0
3325 0
3511 0
3748 0
3936 0
4110 0
4329 0
4564 0
4766 0
5019 0
5233 0
5465 0
5659 0
5868 0
6107 0
6368 0
6581 0
6784 0
6954 0
7118 0
7279 0
7440 0
7656 0
7870 0
8043 0
8232 0
8439 0
8634 0
8816 0
9010 0
9212 0
9390 0
9552 0
9716 0
9894 0
10069 0
10241 0
10416 0
10581 0
10741 0
10901 0
11063 0
11246 0
11436 0
11614 0
11819 0
11992 0
12152 0
12333 13
12548 27
12729 32
12919 35
13113 35
13305 35
13476 35
13679 35
13858 35
14037 35
14229 35
14424 35
14590 35
14783 35
14977 35
15185 35
15371 35
15578 36
15748 36
15916 36
16108 45
16333 96
16577 100
16783 100
17052 102
17303 105
17499 106
17688 106
17896 106
18138 108
18345 108
18552 109
18758 109
18995 110
19260 115
19510 128
19710 128
19960 130
20224 132
20476 134
20682 134
20869 135
21103 137
21328 140
21558 149
21737 149
21914 149
22129 155
22332 156
22578 158
22786 202
22962 378
23129 545
23334 705
23549 853
23788 1092
24031 1335
24225 1529
24391 1695
24558 1862
24740 2044
24920 2224
25096 2400
25268 2572
25428 2732
25590 2894
25752 3056
25915 3219
26081 3385
26243 3547
26406 3710
26571 3875
26745 4049
26916 4220
27086 4390
27248 4552
27423 4727
27604 4908
27788 5092
27968 5272
28145 5449
28334 5638
28522 5826
28714 6018
28887 6191
29062 6366
29224 6528
29396 6700
29574 6878
29744 7048
29913 7217
30092 7396
30275 7579
30453 7757
30635 7939
30814 8118
30995 8299
31189 8493
31380 8684
31575 8879
31760 9064
31931 9235
32116 9420
};
\addlegendentry{default}
\addplot [semithick, color1]
table {%
4 0
232 0
452 0
635 0
838 0
1040 0
1217 0
1380 0
1542 0
1706 0
1882 0
2112 0
2288 0
2463 0
2626 0
2809 0
2997 0
3171 0
3344 0
3540 0
3759 0
3953 0
4130 0
4361 0
4603 0
4809 0
5046 0
5260 0
5498 0
5672 0
5881 0
6105 0
6364 0
6599 0
6791 0
6982 0
7146 0
7306 0
7468 0
7649 0
7890 0
8067 0
8251 0
8446 0
8645 0
8821 0
9006 0
9213 0
9389 0
9550 0
9713 0
9887 0
10065 0
10238 0
10419 0
10591 0
10751 0
10911 0
11073 0
11265 0
11453 0
11635 0
11826 0
11999 0
12159 0
12340 13
12557 27
12738 31
12925 36
13124 36
13330 36
13496 36
13701 36
13893 36
14069 36
14258 36
14437 36
14617 36
14827 36
15021 69
15225 89
15428 89
15606 89
15827 91
15991 91
16158 91
16337 91
16555 93
16808 96
17029 97
17248 98
17465 99
17653 99
17895 101
18137 103
18326 103
18549 104
18779 105
18990 105
19246 107
19480 108
19687 108
19953 123
20165 125
20343 125
20557 126
20808 127
21079 129
21334 130
21576 133
21738 133
21949 134
22170 147
22414 155
22659 164
22836 286
23011 461
23187 637
23354 803
23572 994
23820 1242
24050 1472
24237 1659
24404 1826
24572 1994
24747 2169
24933 2355
25113 2535
25279 2701
25441 2863
25604 3026
25765 3187
25929 3351
26092 3514
26255 3677
26417 3839
26590 4012
26760 4182
26931 4353
27098 4520
27266 4688
27443 4865
27624 5046
27810 5232
27992 5414
28169 5591
28357 5779
28542 5964
28724 6146
28895 6317
29085 6507
29253 6675
29432 6854
29597 7019
29764 7186
29933 7355
30110 7532
30291 7713
30474 7896
30652 8074
30834 8256
31015 8437
31204 8626
31401 8823
31598 9020
31777 9199
31950 9372
32135 9557
32323 9745
32501 9923
};
\addlegendentry{fix-checkmates}
\addplot [semithick, white!67.05882352941175!black]
table {%
5 1
216 37
403 99
603 186
782 207
971 207
1190 207
1416 207
1647 207
1886 207
2124 207
2290 207
2455 207
2626 207
2804 207
2978 207
3144 207
3318 207
3483 207
3644 207
3807 207
3972 207
4146 207
4322 207
4506 207
4687 207
4880 207
5079 207
5260 207
5434 207
5626 207
5842 207
6051 207
6258 207
6467 207
6659 207
6876 210
7065 213
7262 229
7483 243
7697 255
7896 284
8074 382
8235 400
8406 400
8573 400
8735 400
8897 400
9058 400
9258 400
9436 400
9601 400
9762 400
9925 400
10118 400
10342 400
10575 400
10803 413
11043 446
11260 521
11479 532
11694 569
11923 658
12151 886
12400 1135
12579 1314
12764 1499
12924 1659
13085 1820
13273 2008
13479 2214
13679 2414
13889 2624
14088 2823
14307 3042
14497 3232
14675 3410
14876 3611
15077 3812
15237 3972
15399 4134
15568 4303
15735 4470
15902 4637
16064 4799
16228 4963
16392 5127
16564 5299
16732 5467
16903 5638
17067 5802
17228 5963
17396 6131
17561 6296
17724 6459
17889 6624
18060 6795
18228 6963
18394 7129
18562 7297
18733 7468
18910 7645
19090 7825
19261 7996
19441 8176
19617 8352
19786 8521
19954 8689
20129 8864
20308 9043
20494 9229
20682 9417
20867 9602
21040 9775
21226 9961
21407 10142
21586 10321
21779 10514
21983 10718
22175 10910
22363 11098
22555 11290
22747 11482
22942 11677
23123 11858
23318 12053
23493 12228
23682 12417
23869 12604
24058 12793
24257 12992
24451 13186
24653 13388
24854 13589
25043 13778
25235 13970
25409 14144
25593 14328
25787 14522
25970 14705
26158 14893
26348 15083
26530 15265
26700 15435
26869 15604
27040 15775
27211 15946
27380 16115
27550 16285
27720 16455
27883 16618
28054 16789
28221 16956
28386 17121
28558 17293
28721 17456
28893 17628
29060 17795
29234 17969
29410 18145
29582 18317
29747 18482
29918 18653
30095 18830
};
\addlegendentry{enhance-checks}
\addplot [semithick, white!34.90196078431372!black]
table {%
4 0
227 0
435 0
609 0
785 0
977 0
1140 0
1300 0
1463 0
1633 0
1798 0
1970 0
2138 0
2307 0
2479 0
2652 0
2855 0
3049 0
3217 0
3401 0
3572 0
3741 0
3920 7
4086 7
4257 7
4440 20
4645 21
4854 25
5041 25
5242 26
5432 27
5650 27
5833 27
6030 27
6243 28
6469 28
6653 31
6844 31
7022 31
7210 31
7434 32
7635 33
7802 33
7968 33
8130 33
8300 33
8513 33
8747 34
8941 34
9185 35
9400 36
9595 52
9783 78
9969 83
10201 85
10454 87
10704 88
10963 91
11229 92
11505 94
11746 95
11976 97
12233 99
12432 99
12627 99
12857 100
13115 101
13290 101
13506 101
13710 102
13929 116
14167 118
14433 120
14661 121
14853 121
15032 121
15231 121
15464 122
15686 123
15878 123
16108 124
16359 126
16618 138
16859 145
17087 147
17295 241
17466 412
17640 586
17821 754
17987 859
18157 859
18331 859
18496 859
18756 870
18990 876
19165 876
19331 876
19505 876
19771 882
19994 1075
20246 1327
20477 1558
20639 1720
20807 1888
20979 2060
21158 2239
21332 2413
21492 2573
21655 2736
21817 2898
21979 3060
22146 3227
22310 3391
22473 3554
22636 3717
22809 3890
22983 4064
23165 4246
23336 4417
23503 4584
23681 4762
23865 4946
24056 5137
24240 5321
24417 5498
24606 5687
24799 5880
24983 6064
25173 6254
25364 6445
25554 6635
25744 6825
25944 7025
26119 7200
26311 7392
26519 7600
26706 7787
26883 7964
27058 8139
27253 8334
27432 8513
27606 8687
27778 8859
27944 9025
28131 9212
28327 9408
28497 9578
28683 9764
28855 9936
29047 10128
29228 10309
29422 10503
29606 10687
29784 10865
29977 11058
30155 11236
30356 11437
30550 11631
30740 11821
30928 12009
31113 12194
31300 12381
31477 12558
31659 12740
31852 12933
32032 13113
32225 13306
32401 13482
};
\addlegendentry{u-value-exploration-factor}
\addplot [semithick, color2]
table {%
5 1
216 37
404 101
593 162
771 163
948 165
1113 165
1273 165
1435 165
1596 165
1758 165
1923 165
2089 165
2252 165
2419 165
2592 165
2760 165
2930 165
3098 165
3268 165
3445 165
3635 165
3827 165
4012 165
4190 165
4366 165
4533 165
4697 165
4857 165
5019 165
5187 165
5349 165
5516 165
5682 165
5847 165
6019 165
6193 165
6365 165
6527 165
6694 165
6864 165
7037 165
7216 165
7386 165
7570 165
7740 165
7934 165
8161 165
8378 165
8550 165
8730 165
8920 165
9135 165
9377 165
9614 165
9842 165
10087 171
10337 182
10592 191
10827 191
11053 191
11297 191
11532 191
11758 191
11926 191
12094 191
12272 191
12467 191
12640 191
12833 191
13022 191
13228 192
13473 198
13709 200
13882 200
14048 200
14214 200
14473 217
14734 221
14986 232
15236 234
15422 235
15582 235
15756 236
16010 240
16262 253
16521 273
16726 374
16948 399
17180 407
17403 421
17651 461
17878 501
18131 513
18390 522
18638 537
18885 579
19098 582
19330 748
19576 994
19808 1226
19985 1403
20155 1573
20316 1734
20479 1897
20688 2106
20886 2304
21095 2513
21310 2728
21513 2931
21704 3122
21887 3305
22061 3479
22224 3642
22429 3847
22632 4050
22821 4239
23003 4421
23207 4625
23388 4806
23550 4968
23716 5134
23879 5297
24041 5459
24205 5623
24371 5789
24537 5955
24706 6124
24876 6294
25046 6464
25208 6626
25377 6795
25545 6963
25714 7132
25887 7305
26057 7475
26228 7646
26400 7818
26575 7993
26747 8165
26917 8335
27086 8504
27252 8670
27431 8849
27625 9043
27811 9229
28011 9429
28210 9628
28388 9806
28572 9990
28752 10170
28951 10369
29132 10550
29321 10739
29504 10922
29686 11104
29874 11292
30062 11480
30239 11657
30430 11848
};
\addlegendentry{all}
\end{axis}

\end{tikzpicture}

==> latex_figures/eval_cpu_openings_f.tex <==
\ifarxiv
\def\boardwidth{0.199}
\else
\def\boardwidth{0.195}
\fi
\begin{figure}
\centering
\begin{minipage}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=rnbqkbnr/pppp1ppp/8/4p3/4P3/8/PPPP1PPP/RNBQKBNR/ w KQkq - 2 2,]
}
\caption*{\csmall{C20 King's Pawn Game}}
%\caption{\csmall{C20 King's Pawn Game}}
\end{minipage}
%
\begin{minipage}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=rnbqkbnr/pppp1ppp/4p3/8/4P3/8/PPPP1PPP/RNBQKBNR/ w KQkq - 2 2,]
}
\caption*{\csmall{C00 French Defense}}
\end{minipage}%
%
\begin{minipage}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=rnbqkb1r/pppppppp/5n2/8/4P3/8/PPPP1PPP/RNBQKBNR/ w KQkq - 2 2,]
}
\caption*{\csmall{B02 Alekhine Defense}}
\end{minipage}%
%
\begin{minipage}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=rnbqkbnr/ppp1pppp/3p4/8/4P3/8/PPPP1PPP/RNBQKBNR/ w KQkq - 2 2,]
}
\caption*{\csmall{B07 Pirc Defense}}
\end{minipage}%
%
\begin{minipage}{\boardwidth\textwidth}
\vspace{0.37cm}
\resizebox{\textwidth}{!}{
\chessboard[setfen=rnbqkbnr/ppp1pppp/8/3p4/3P4/8/PPP1PPPP/RNBQKBNR/ w KQkq - 2 2,]
}
\caption*{\csmall{D00 Queen's Pawn\\Game}}
\end{minipage}%
\caption{Chosen opening positions validating the playing strength of \alg{CrazyAra 0.6.0} on CPU}
\label{fig:openings_cpu}
\end{figure}
%\addtocounter{subfigure}{-5}

==> latex_figures/eval_gpu_openings_f.tex <==
\begin{figure}
\centering
\begin{subfigure}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=r1bqkbnr/pppp1ppp/2n5/1B2p3/4P3/5N2/PPPP1PPP/RNBQK2R b KQkq - 3 3,]
}
\caption*{\csmall{A00 Hungarian Opening}}
\end{subfigure}
%
\begin{subfigure}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=r1bq1rk1/ppppbppp/2n2n2/4p1B1/2B1P3/3P1N2/PPP2PPP/RN1Q1RK1 w - - 3 7,]
}
\caption*{\csmall{C50 Giuoco Piano}}
\end{subfigure}%
%
\begin{subfigure}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
%\vspace{-13.5cm}
%\vspace{-0.5cm}
%\chessboard[setfen=rnbqkb1r/ppp2ppp/5p2/3p4/8/8/PPPP1PPP/RNBQKBNR/Np w KQkq - 6 4,] -> previously used in cafish 0.4.1
\chessboard[
% Pocket pieces
pgfstyle={text},
text=\;\qquad\WhiteKnightOnWhite,
markfield={h8},
text=\;\qquad\BlackPawnOnWhite, 
markfield={h7},
%
setfen=r1bqkb1r/ppp2ppp/2n2p2/3p4/3P4/8/PPP2PPP/RNBQKBNR/Np w KQkq - 2 5,]
}
\caption*{\csmall{B02 Crosky Gambit %\resizebox{0.17\textwidth}{!}{\WhiteKnightOnWhite \BlackPawnOnWhite}
}}
\end{subfigure}%
%
\begin{subfigure}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=rn1qkbnr/ppp1pppp/8/3p1b2/3P4/4P3/PPP2PPP/RNBQKBNR w KQkq - 1 3,]
}
\caption*{\csmall{B02 Crosky Gambit %\resizebox{0.17\textwidth}{!}{\WhiteKnightOnWhite \BlackPawnOnWhite}
}}
\end{subfigure}%
%
\begin{subfigure}{\boardwidth\textwidth}
\resizebox{\textwidth}{!}{
\chessboard[setfen=rnbqkb1r/ppp1pppp/5n2/3p4/3P4/6P1/PPP1PPBP/RNBQK1NR b KQkq - 2 3,]
}
\caption*{\csmall{A00 Hungarian Opening}}
\end{subfigure}%
\caption{Chosen opening positions between \alg{CrazyAraFish 0.6.0} on GPU and \alg{Stockfish 10}}
\label{fig:openings_gpu}
\end{figure}
%\addtocounter{subfigure}{-5}

==> latex_figures/mcts_tactic_pos.tex <==
\begin{figure}
\centering
\begin{minipage}{.49\textwidth}
%
\centering
\input{chessboards/tactic_pos.tex}
\caption{Exemplary tactical board position}
\label{fig:tactical_board}
%
%
\end{minipage}%
\hfill
\begin{minipage}{0.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/demo_prediction/policy_distribution_tactic_pos.pdf}
  \captionof{figure}{Sorted policy distribution of the first ten candidate moves}% (\textit{(probably move this figure to the supplementary materials)}}
  \label{fig:candidate_moves}
  \label{fig:test2}
  \vspace{1cm}
\end{minipage}
\end{figure}

==> pgn/CrazyAraFish041_SF10/10_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "5"]
[White "stockfish-x86_64-modern  2018-11-29"]
[Black "CrazyAraFish-Dev-0.4.1-Rise"]
[Result "1-0"]
[PlyCount "69"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}

\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{Stockfish 10 x86\_64-modern  2018-11-29}
 Black: \textit{CrazyAraFish-0.4.1} Result: \textit{1-0}  TimeControl 40/1800 PlyCount 69
 
1. g3 \{book\} d5 \{book\} 2. d4 \{book\} Nf6 \{book\} 3. Bg2 \{book\} Bf5 \{-0.15/30 37s\}
4. Nc3 \{+0.05/28 106s\} Nc6 \{-0.26/32 37s\} 5. Nf3 \{0.00/28 19s\} e6 \{-0.22/28 37s\}
6. O-O \{-0.13/29 79s\} Be7 \{-0.12/29 37s\} 7. Ne5 \{0.00/27 14s\} O-O \{+0.74/25 47s\}
8. Nxc6 \{+0.54/26 14s\} bxc6 \{+0.93/25 47s\} 9. N@e5 \{-0.81/28 273s\}
Qd6 \{+0.92/22 46s\} 10. h3 \{-0.16/26 19s\} Rab8 \{+0.81/23 46s\}
11. a3 \{+0.66/26 24s\} Kh8 \{+0.99/21 46s\} 12. g4 \{+1.46/24 24s\}
Bg6 \{+0.47/29 49s\} 13. Nxg6+ \{+1.21/24 25s\} fxg6 \{+2.27/19 47s\}
14. B@e5 \{+2.02/24 26s\} N@h4 \{+2.44/33 49s\} 15. Nxd5 \{+5.26/23 18s\}
exd5 \{-2.14/25 49s\} 16. P@h6 \{+5.65/23 31s\} N@e8 \{-1.19/34 50s\}
17. hxg7+ \{+7.53/27 89s\} Nxg7 \{-1.54/31 49s\} 18. Bxd6 \{+7.80/24 13s\}
Bxd6 \{-1.24/25 49s\} 19. P@e5 \{+8.73/24 16s\} B@e4 \{-1.72/23 49s\}
20. Bh6 \{+9.02/22 19s\} N@e6 \{-2.90/24 49s\} 21. f3 \{+9.87/23 23s\}
Nxg2 \{-0.23/34 51s\} 22. Kxg2 \{+10.42/22 27s\} B@g5 \{-0.74/35 49s\}
23. Bxg5 \{+12.97/22 17s\} Nxg5 \{-1.16/30 51s\} 24. exf6 \{+14.47/24 42s\}
Rxf6 \{-4.29/24 50s\} 25. B@e5 \{+15.19/24 29s\} Rbf8 \{-4.52/21 49s\}
26. Bxf6 \{+31.36/22 18s\} Rxf6 \{-7.80/24 48s\} 27. R@g8+ \{+M33/22 19s\}
Kxg8 \{+6.52/1 0.023s\} 28. N@h6+ \{+M27/26 23s\} Kf8 \{-1.20/27 46s\}
29. Q@h8+ \{+M25/28 49s\} Ke7 \{-7.40/23 39s\} 30. Ng8+ \{+M23/30 59s\}
Ke6 \{-12.35/19 40s\} 31. N@d8+ \{+M9/44 22s\} Kd7 \{-15.59/1 0.009s\}
32. Nxf6+ \{+M7/51 31s\} Kc8 \{-17.27/19 29s\} 33. Nxc6+ \{+M5/59 266s\}
Kb7 \{-19.83/14 23s\} 34. Qb8+ \{+M3/91 28s\} Ka6 \{-69.19/2 12s\}
35. P@b5\# \{+M1/127 0.019s, White mates\} 1-0


==> pgn/CrazyAraFish041_SF10/1_cafish_sf10.tex <==
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAraFish-0.4.1} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{1-0}  TimeControl 40/1800 PlyCount 127

1. e4 \{book\} e5 \{book\} 2. Nf3 \{book\} Nc6 \{book\} 3. Bb5 \{book\} Bc5 \{0.00/28 88s\}
4. O-O \{+2.62/38 38s\} Nf6 \{0.00/29 18s\} 5. Nc3 \{+2.16/39 38s\} O-O \{-1.32/28 92s\}
6. d3 \{+1.76/28 38s\} d6 \{-0.25/27 57s\} 7. Bg5 \{+2.69/34 38s\} Nb4 \{-3.03/27 160s\}
8. Na4 \{+3.56/25 47s\} Nxc2 \{-4.48/27 125s\} 9. Nxc5 \{+3.71/35 48s\}
P@h3 \{-3.97/26 35s\} 10. Nxb7 \{+4.21/24 47s\} Bxb7 \{-4.65/26 35s\}
11. gxh3 \{+4.02/25 48s\} Nxa1 \{-4.48/25 21s\} 12. P@g2 \{+4.15/20 46s\}
R@g6 \{-3.38/27 187s\} 13. B@e3 \{+4.44/23 47s\} Kh8 \{-5.63/27 194s\}
14. Qxa1 \{+2.68/21 47s\} N@f4 \{-2.71/24 18s\} 15. Bexf4 \{+3.19/30 50s\}
exf4 \{-2.37/24 15s\} 16. N@h4 \{+3.33/27 49s\} Rxg5 \{-2.25/24 11s\}
17. Nxg5 \{+3.30/34 51s\} Nxe4 \{-1.48/25 22s\} 18. Nxf7+ \{+3.73/34 51s\}
Rxf7 \{-0.84/23 18s\} 19. N@g6+ \{+3.62/34 51s\} hxg6 \{-5.51/25 40s\}
20. Nxg6+ \{+3.71/30 51s\} Kh7 \{-3.86/23 26s\} 21. dxe4 \{+4.10/32 51s\}
Qg5 \{-9.59/26 169s\} 22. N@f3 \{+3.70/26 50s\} Qxb5 \{0.00/21 19s\}
23. P@f5 \{+4.27/28 51s\} Rxf5 \{0.00/23 23s\} 24. exf5 \{+3.67/23 50s\}
Bxf3 \{-3.66/24 76s\} 25. P@e2 \{+4.61/31 51s\} B@f7 \{-2.69/21 14s\}
26. gxf3 \{+5.61/23 51s\} Qxf5 \{-4.64/22 36s\} 27. B@e4 \{+6.10/23 51s\}
Qxg6+ \{-8.43/23 63s\} 28. Bxg6+ \{+6.62/19 49s\} Bxg6 \{-6.56/21 14s\}
29. R@g5 \{+7.61/22 51s\} B@f7 \{-9.58/24 87s\} 30. P@h5 \{+7.84/21 51s\}
Bxh5 \{-8.90/22 14s\} 31. Qb1+ \{+10.69/22 51s\} B@g6 \{-6.20/18 8.9s\}
32. Rxh5+ \{+11.12/21 50s\} P@h6 \{-18.13/19 25s\} 33. B@e4 \{+12.10/21 50s\}
N@e7 \{-23.99/17 37s\} 34. R@g4 \{+14.22/20 50s\} P@g2 \{-8.58/16 5.4s\}
35. Rxg2 \{+16.02/20 50s\} P@g3 \{-9.62/17 5.8s\} 36. hxg3 \{+14.40/18 50s\}
N@d4 \{-12.62/17 18s\} 37. P@f6 \{+16.14/16 49s\} B@f5 \{-15.08/15 11s\}
38. fxe7 \{+16.89/16 40s\} N@e5 \{-21.10/15 5.9s\} 39. Bxf5 \{+21.94/19 40s\}
N@e6 \{-27.26/16 3.2s\} 40. gxf4 \{+21.92/14 40s\} Nxf5 \{-30.44/13 1.8s\}
41. fxe5 \{+23.24/13 46s\} P@h2+ \{-43.64/20 289s\} 42. Kxh2 \{+24.02/14 46s\}
B@f4+ \{-36.98/17 30s\} 43. Kh1 \{+22.05/15 46s\} Nxe7 \{-48.16/19 128s\}
44. P@f5 \{+22.21/14 46s\} Nxf5 \{-60.74/21 368s\} 45. Rxf5 \{+23.12/15 46s\}
Bg5 \{-M38/19 90s\} 46. Rxf7 \{+24.54/18 46s\} P@c2 \{-M36/18 23s\}
47. Qxc2 \{+23.51/16 46s\} Bxc2 \{-M20/20 37s\} 48. Rxg7+ \{+18.92/17 46s\}
Nxg7 \{-47.44/17 16s\} 49. N@f6+ \{+19.09/16 46s\} Bxf6 \{-42.74/16 14s\}
50. exf6 \{+19.27/16 46s\} R@h2+ \{-54.79/19 225s\} 51. Kxh2 \{+26.34/16 46s\}
Q@e5+ \{-51.53/17 69s\} 52. Kh1 \{+26.26/14 46s\} N@g3+ \{-M20/19 83s\}
53. Rxg3 \{+27.30/17 46s\} Qxf6 \{-M18/24 7.8s\} 54. N@d7 \{+28.49/15 46s\}
P@g2+ \{-M14/30 19s\} 55. Rxg2 \{+30.03/18 45s\} Qe6 \{-M14/28 6.5s\}
56. N@f6+ \{+42.31/17 46s\} Kh8 \{-M12/33 9.4s\} 57. P@e4 \{+24.22/18 46s\}
Qxh3+ \{-M12/43 19s\} 58. R@h2 \{+32.38/18 39s\} Qxh2+ \{-M10/53 11s\}
59. Rxh2 \{+34.28/17 32s\} P@g2+ \{-M8/55 11s\} 60. Rxg2 \{+39.63/18 31s\}
R@h3+ \{-M6/65 10s\} 61. P@h2 \{+50.68/9 19s\} Rxh2+ \{-M6/80 9.0s\}
62. Rxh2 \{+56.10/15 21s\} P@g2+ \{-M4/93 11s\} 63. Rxg2 \{+57.40/8 14s\}
d5 \{-M2/110 35s\} 64. N@f7\# \{+M1/1 11s, White mates\} 1-0


==> pgn/CrazyAraFish041_SF10/2_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "1"]
[White "stockfish-x86_64-modern  2018-11-29"]
[Black "CrazyAraFish-Dev-0.4.1-Rise"]
[Result "1-0"]
[PlyCount "105"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{Stockfish 10 x86\_64-modern  2018-11-29}
 Black: \textit{CrazyAraFish-0.4.1} Result: \textit{1-0}  TimeControl 40/1800 PlyCount 105

1. e4 \{book\} e5 \{book\} 2. Nf3 \{book\} Nc6 \{book\} 3. Bb5 \{book\} Nf6 \{-1.02/37 37s\}
4. Nc3 \{+1.83/28 140s\} Be7 \{-1.41/35 37s\} 5. Nxe5 \{+1.85/25 36s\}
Nxe5 \{-1.10/28 37s\} 6. d4 \{+2.37/25 30s\} Ng6 \{-0.69/27 37s\} 7. e5 \{+2.04/26 46s\}
O-O \{-1.77/26 47s\} 8. P@h6 \{+1.77/27 92s\} d6 \{-2.34/29 49s\}
9. hxg7 \{+2.25/25 38s\} dxe5 \{-2.10/26 48s\} 10. Bg5 \{+2.55/24 27s\}
P@h3 \{-0.37/28 49s\} 11. Bxf6 \{+1.94/24 34s\} Bxf6 \{-0.07/34 48s\}
12. gxf8=Q+ \{+1.95/25 101s\} Qxf8 \{-0.27/26 48s\} 13. Ne4 \{+1.99/23 14s\}
hxg2 \{+2.03/31 48s\} 14. Nxf6+ \{-1.00/22 55s\} Kh8 \{+2.14/29 48s\}
15. Rg1 \{+0.73/22 26s\} P@e3 \{+3.07/28 48s\} 16. Qe2 \{0.00/24 111s\}
exf2+ \{+1.84/26 48s\} 17. Qxf2 \{+1.53/22 12s\} B@h4 \{+2.01/28 48s\}
18. O-O-O \{0.00/23 97s\} Bxf2 \{-0.57/26 48s\} 19. R@e8 \{+1.83/21 13s\}
Q@g7 \{-0.74/37 48s\} 20. B@g5 \{+2.56/26 234s\} P@a3 \{-0.47/35 52s\}
21. P@h6 \{+10.08/25 11s\} axb2+ \{-0.20/34 48s\} 22. Kb1 \{+8.07/27 100s\}
N@c3+ \{-4.00/26 48s\} 23. Kxb2 \{+2.28/1 0s\} Nxd1+ \{-5.67/25 50s\}
24. Rxd1 \{+10.75/24 10.0s\} Bxd4+ \{-5.39/24 50s\} 25. P@c3 \{+10.79/26 40s\}
Bxc3+ \{-6.04/31 52s\} 26. Kxc3 \{+13.91/24 46s\} P@b4+ \{-5.06/23 51s\}
27. Kb2 \{+6.68/25 51s\} P@c3+ \{-5.52/31 51s\} 28. Kb1 \{+6.62/24 22s\}
R@b2+ \{-5.43/27 51s\} 29. Ka1 \{+9.97/24 12s\} Rxa2+ \{-4.59/28 51s\}
30. Kxa2 \{+11.32/25 48s\} Be6+ \{-5.44/25 51s\} 31. Rxe6 \{+12.31/23 12s\}
fxe6 \{-3.90/24 51s\} 32. hxg7+ \{+14.76/25 140s\} Qxg7 \{-5.01/20 26s\}
33. B@a3 \{+15.92/19 5.8s\} P@b3+ \{-6.46/21 55s\} 34. Kxb3 \{+17.39/21 60s\}
P@a4+ \{-4.13/23 51s\} 35. Bxa4 \{+22.25/19 11s\} bxa3 \{-4.79/27 49s\}
36. P@h6 \{+24.12/21 18s\} R@b2+ \{-3.97/23 46s\} 37. Kxc3 \{+27.63/20 36s\}
B@b4+ \{-3.58/29 48s\} 38. Kd3 \{+29.66/20 11s\} Rd8+ \{-3.60/24 34s\}
39. Ke2 \{+36.77/21 11s\} Nf4+ \{-7.52/21 36s\} 40. Bxf4 \{+59.18/23 48s\}
Rd2+ \{-9.04/20 35s\} 41. Bxd2 \{+M27/24 48s\} P@f3+ \{-11.06/21 50s\}
42. Kd3 \{+M25/27 44s\} e4+ \{-11.82/19 51s\} 43. Nxe4 \{+M23/28 38s\}
P@c4+ \{-13.68/21 51s\} 44. Kxc4 \{+M21/30 49s\} Rxc2+ \{-14.69/19 51s\}
45. Bxc2 \{+M19/30 41s\} b5+ \{-16.22/19 51s\} 46. Kxb4 \{+M17/34 36s\}
Qd4+ \{-18.47/16 50s\} 47. Kxa3 \{+M15/43 32s\} b4+ \{-23.41/17 42s\}
48. Bxb4 \{+M13/46 30s\} Qxb4+ \{-24.40/16 45s\} 49. Kxb4 \{+M11/54 54s\}
B@f8+ \{-26.22/14 46s\} 50. Kb3 \{+M9/48 41s\} P@a4+ \{-32.20/10 45s\}
51. Kxa4 \{+M7/91 29s\} Bxh6 \{-36.54/12 38s\} 52. Q@e8+ \{+M3/97 45s\}
Kg7 \{-86.10/10 17s\} 53. Q@f7\# \{+M1/126 0.039s, White mates\} 1-0


==> pgn/CrazyAraFish041_SF10/3_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "2"]
[White "CrazyAraFish-Dev-0.4.1-Rise"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "0-1"]
[PlyCount "90"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAraFish-0.4.1} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{0-1}  TimeControl 40/1800 PlyCount 90

1. e4 \{book\} e5 \{book\} 2. Nf3 \{book\} Nc6 \{book\} 3. Bc4 \{book\} Bc5 \{book\}
4. O-O \{book\} Nf6 \{book\} 5. d3 \{book\} O-O \{book\} 6. Bg5 \{book\} Be7 \{book\}
7. d4 \{+0.37/27 41s\} exd4 \{+1.68/27 78s\} 8. e5 \{+0.45/28 41s\} Ng4 \{+2.57/25 23s\}
9. Bxe7 \{+0.65/28 41s\} Qxe7 \{+3.26/24 11s\} 10. B@h4 \{+0.45/32 41s\}
Qc5 \{+1.64/27 304s\} 11. Nbd2 \{+0.57/29 49s\} B@f4 \{+1.83/26 22s\}
12. Bd3 \{+0.54/28 49s\} d5 \{+2.88/25 17s\} 13. exd6 \{+0.38/26 49s\}
Qxd6 \{+0.52/28 266s\} 14. Ne4 \{+0.85/28 51s\} Qg6 \{+0.69/27 116s\}
15. P@f6 \{+1.79/22 49s\} P@f5 \{+1.27/26 69s\} 16. fxg7 \{+1.64/30 51s\}
Qxg7 \{0.00/26 33s\} 17. P@f6 \{+1.50/22 49s\} Qh6 \{+3.61/24 24s\}
18. Ng3 \{+1.32/33 52s\} P@e3 \{+2.28/25 99s\} 19. fxe3 \{+1.55/32 50s\}
Bxe3+ \{+4.92/26 31s\} 20. Kh1 \{+0.74/38 53s\} P@e4 \{+5.82/26 15s\}
21. Bxe4 \{+1.47/28 50s\} fxe4 \{+6.01/26 18s\} 22. Nxe4 \{+0.49/37 52s\}
Re8 \{+6.45/26 52s\} 23. P@g5 \{+1.87/24 51s\} Qg6 \{+7.35/23 7.8s\}
24. P@d3 \{+0.94/30 51s\} P@h3 \{+10.85/23 14s\} 25. Qe2 \{-1.22/31 52s\}
hxg2+ \{+20.01/24 29s\} 26. Qxg2 \{-2.64/32 53s\} P@h3 \{+21.30/24 14s\}
27. Qxh3 \{+2.07/32 54s\} Rxe4 \{+21.49/25 27s\} 28. dxe4 \{-4.33/26 51s\}
Nf2+ \{+23.64/24 17s\} 29. Rxf2 \{-6.55/23 51s\} Bxh3 \{+26.44/24 35s\}
30. N@f4 \{-6.92/27 52s\} Bxf4 \{+27.21/25 21s\} 31. P@g2 \{-7.11/26 54s\}
Bxg2+ \{+30.08/23 49s\} 32. Rxg2 \{-8.78/28 52s\} P@h3 \{+30.62/23 34s\}
33. B@f1 \{-8.11/24 55s\} hxg2+ \{+31.49/21 50s\} 34. Bxg2 \{-9.32/24 51s\}
Q@g4 \{+32.66/23 78s\} 35. R@f2 \{-8.63/21 53s\} Bxh2 \{+32.92/21 67s\}
36. P@h3 \{-9.81/20 53s\} Q4xe4 \{+33.03/19 17s\} 37. P@f5 \{-9.50/16 53s\}
Qgxf5 \{+38.79/19 32s\} 38. P@g4 \{-10.75/22 51s\} Qff4 \{+50.62/19 19s\}
39. Nxh2 \{-13.11/25 48s\} Qxf2 \{+M15/37 17s\} 40. Bxf2 \{-15.27/23 42s\}
Qxg2+ \{+M11/49 36s\} 41. Kxg2 \{-18.11/1 0.026s\} N@f4+ \{+M9/59 36s\}
42. Kg3 \{-14.79/17 42s\} N@e2+ \{+M7/63 33s\} 43. Kh4 \{-18.18/17 22s\}
R@h5+ \{+M5/92 33s\} 44. gxh5 \{-7.85/1 0.023s\} Ng2+ \{+M3/127 1.1s\}
45. Kg4 \{-20.58/1 0.015s\} R@f4\# \{+M1/127 0.020s, Black mates\} 0-1


==> pgn/CrazyAraFish041_SF10/4_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "2"]
[White "stockfish-x86_64-modern  2018-11-29"]
[Black "CrazyAraFish-Dev-0.4.1-Rise"]
[Result "1-0"]
[PlyCount "63"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{Stockfish 10 x86\_64-modern  2018-11-29}
 Black: \textit{CrazyAraFish-0.4.1} Result: \textit{1-0}  TimeControl 40/1800 PlyCount 63
 
1. e4 \{book\} e5 \{book\} 2. Nf3 \{book\} Nc6 \{book\} 3. Bc4 \{book\} Bc5 \{book\}
4. O-O \{book\} Nf6 \{book\} 5. d3 \{book\} O-O \{book\} 6. Bg5 \{book\} Be7 \{book\}
7. Be3 \{+2.75/27 72s\} d6 \{+0.06/27 41s\} 8. Ng5 \{+0.59/29 71s\} d5 \{+0.13/27 41s\}
9. exd5 \{-0.09/28 45s\} Nxd5 \{+0.06/24 41s\} 10. Qh5 \{+0.37/27 30s\}
Bxg5 \{+0.56/30 41s\} 11. Bxg5 \{+1.31/28 35s\} N@e2+ \{+0.84/28 49s\}
12. Kh1 \{+3.77/26 26s\} P@h3 \{+0.52/33 50s\} 13. B@e4 \{+3.76/26 24s\}
hxg2+ \{+0.84/31 49s\} 14. Bxg2 \{+4.68/28 16s\} Nf6 \{+0.35/31 49s\}
15. Qxe2 \{+4.13/29 198s\} P@h3 \{+0.68/28 48s\} 16. Bxc6 \{+6.05/25 28s\}
bxc6 \{+0.53/33 50s\} 17. Kg1 \{+6.28/24 47s\} Bg4 \{+0.77/31 49s\}
18. f3 \{+8.03/21 11s\} B@g2 \{+0.94/33 49s\} 19. N@e4 \{+10.51/25 205s\}
Bxf1 \{-0.42/30 48s\} 20. Nxf6+ \{+11.37/23 18s\} Kh8 \{+0.54/36 45s\}
21. P@h6 \{+23.72/22 19s\} Rg8 \{-1.81/24 46s\} 22. N@g6+ \{+35.89/24 46s\}
hxg6 \{-7.30/25 32s\} 23. hxg7+ \{+36.25/21 20s\} Rxg7 \{-7.24/22 33s\}
24. P@h6 \{+39.94/22 14s\} Qd4+ \{-8.73/22 45s\} 25. N@e3 \{+46.38/23 19s\}
N@h7 \{-8.99/22 45s\} 26. hxg7+ \{+M25/21 17s\} Kxg7 \{-9.27/1 0.020s\}
27. Nxg4 \{+M19/30 39s\} Nxg5 \{-11.80/22 45s\} 28. B@f6+ \{+M9/44 63s\}
Kf8 \{-16.06/16 27s\} 29. P@e7+ \{+M7/45 32s\} Ke8 \{-16.76/21 27s\}
30. R@f8+ \{+M5/63 23s\} Kd7 \{-13.40/1 0.019s\} 31. Rd8+ \{+M3/83 26s\}
Rxd8 \{-39.84/1 0.009s\} 32. exd8=Q\# \{+M1/127 0.006s, White mates\} 1-0


==> pgn/CrazyAraFish041_SF10/5_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "3"]
[White "CrazyAraFish-Dev-0.4.1-Rise"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "0-1"]
[PlyCount "102"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}

\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAraFish-0.4.1} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{0-1}  TimeControl 40/1800 PlyCount 102

1. e4 \{book\} Nf6 \{book\} 2. e5 \{book\} d5 \{book\} 3. exf6 \{book\} exf6 \{book\}
4. Bb5+ \{+1.36/28 38s\} c6 \{+0.75/28 75s\} 5. Be2 \{+1.87/22 38s\}
Bd6 \{+0.90/26 12s\} 6. d4 \{+2.10/20 38s\} O-O \{+1.09/26 21s\} 7. Nc3 \{+1.86/25 38s\}
Re8 \{-0.09/32 280s\} 8. Nf3 \{+1.31/25 47s\} Na6 \{-0.48/31 59s\}
9. N@h5 \{+2.07/23 46s\} Bf8 \{-0.52/27 34s\} 10. O-O \{+1.87/21 46s\}
P@h3 \{-0.35/27 14s\} 11. gxh3 \{+2.13/27 47s\} Bxh3 \{+0.21/26 24s\}
12. Nf4 \{+2.29/18 46s\} Bd7 \{0.00/30 136s\} 13. P@g2 \{+1.47/19 46s\}
Nc7 \{-0.16/28 192s\} 14. Kh1 \{+2.59/18 45s\} Bg4 \{0.00/26 20s\}
15. Be3 \{+2.80/23 46s\} Bd6 \{0.00/25 13s\} 16. Nh4 \{+2.99/22 48s\}
Bxe2 \{-0.86/26 45s\} 17. Ncxe2 \{+3.01/26 49s\} B@e4 \{-1.23/28 86s\}
18. f3 \{+3.56/24 49s\} Bxf3 \{+1.25/24 14s\} 19. Rxf3 \{+0.42/26 51s\}
Rxe3 \{+2.52/26 17s\} 20. B@h5 \{+0.87/28 50s\} Rxf3 \{+8.74/22 10s\}
21. Bxf7+ \{+0.40/29 51s\} Kxf7 \{+4.84/25 78s\} 22. Nxf3 \{+0.42/25 51s\}
Bxf4 \{+4.85/23 26s\} 23. Qf1 \{+0.48/26 51s\} B@e3 \{+4.16/22 75s\}
24. P@f2 \{+0.43/23 51s\} Kg8 \{+9.28/22 23s\} 25. fxe3 \{+0.05/28 50s\}
Bxe3 \{+8.93/23 33s\} 26. B@f4 \{+0.08/26 51s\} Bxf4 \{+9.29/25 45s\}
27. Nxf4 \{-0.36/27 52s\} B@e3 \{+8.62/25 62s\} 28. B@f7+ \{-0.41/25 52s\}
Kh8 \{+9.48/25 35s\} 29. B@e8 \{-1.06/23 52s\} R@f8 \{+11.37/25 11s\}
30. Nh4 \{-0.96/26 53s\} Bxf4 \{+12.50/26 37s\} 31. Qxf4 \{-0.61/30 51s\}
B@e4 \{+13.57/25 11s\} 32. B@f5 \{-1.20/30 52s\} Bxf5 \{+16.27/21 11s\}
33. Nxf5 \{-0.45/32 52s\} N@h3 \{+20.70/24 52s\} 34. gxh3 \{-4.30/26 52s\}
B@e4+ \{+21.21/22 20s\} 35. B@g2 \{-5.38/28 51s\} Bxg2+ \{+21.86/21 16s\}
36. Kxg2 \{-5.70/27 52s\} B@e4+ \{+22.82/21 15s\} 37. B@f3 \{-6.72/27 50s\}
Bxf3+ \{+23.32/20 14s\} 38. Kxf3 \{-5.88/24 39s\} B@e4+ \{+25.00/22 39s\}
39. Kf2 \{-7.50/23 39s\} Bxf5 \{+25.87/21 44s\} 40. Qxf5 \{-7.34/21 40s\}
N@e4+ \{+38.04/21 33s\} 41. Ke3 \{-9.19/22 51s\} P@f4+ \{+46.69/24 27s\}
42. Kd3 \{-10.12/22 51s\} P@c4+ \{+58.44/23 30s\} 43. Ke2 \{-11.72/1 0.031s\}
P@f3+ \{+M35/25 32s\} 44. Kxf3 \{-14.55/20 49s\} N@h4+ \{+M15/29 27s\}
45. Ke2 \{-19.75/18 45s\} Nxf5 \{+M13/34 44s\} 46. N@g6+ \{-29.52/16 46s\}
hxg6 \{+M11/1 0s\} 47. R@h7+ \{-30.33/14 45s\} Kxh7 \{+M9/1 0s\}
48. Bxg6+ \{-34.04/17 42s\} Kh8 \{+M7/53 139s\} 49. B@e3 \{-24.71/16 46s\}
R@d2+ \{+M5/64 446s\} 50. Bxd2 \{-22.35/14 29s\} Q@f2+ \{+M3/77 29s\}
51. Kd1 \{-32.66/1 0.023s\} Qxd2\# \{+M1/127 0.015s, Black mates\} 0-1


==> pgn/CrazyAraFish041_SF10/6_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "3"]
[White "stockfish-x86_64-modern  2018-11-29"]
[Black "CrazyAraFish-Dev-0.4.1-Rise"]
[Result "1-0"]
[PlyCount "39"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}

\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{Stockfish 10 x86\_64-modern  2018-11-29}
 Black: \textit{CrazyAraFish-0.4.1} Result: \textit{1-0}  TimeControl 40/1800 PlyCount 39

1. e4 \{book\} Nf6 \{book\} 2. e5 \{book\} d5 \{book\} 3. exf6 \{book\} exf6 \{book\}
4. Nc3 \{+0.23/30 92s\} d4 \{-0.57/27 38s\} 5. Bb5+ \{+0.73/26 10s\}
Nc6 \{-1.15/31 38s\} 6. Qe2+ \{0.00/30 273s\} Be7 \{-1.49/25 38s\}
7. N@a5 \{+1.75/27 27s\} Qd7 \{-1.50/28 38s\} 8. Nf3 \{0.00/30 45s\}
P@h3 \{+0.02/31 47s\} 9. Nxd4 \{+2.91/26 72s\} hxg2 \{-1.40/34 47s\}
10. Rg1 \{+3.23/23 10s\} Nxd4 \{-1.85/29 47s\} 11. Bxd7+ \{+15.99/23 36s\}
Bxd7 \{-4.20/32 46s\} 12. Qxe7+ \{+M17/28 33s\} Kxe7 \{+9.65/1 0.027s\}
13. Nd5+ \{+M15/41 19s\} Kf8 \{-4.16/28 44s\} 14. P@e7+ \{+M13/48 15s\}
Ke8 \{-6.59/31 43s\} 15. Q@f8+ \{+M11/55 16s\} Rxf8 \{-1.06/1 0.014s\}
16. exf8=Q+ \{+M9/56 41s\} Kxf8 \{+9.51/1 0.025s\} 17. R@h8+ \{+M7/57 44s\}
B@g8 \{-16.05/13 17s\} 18. B@e7+ \{+M5/56 63s\} Ke8 \{-19.72/1 0.006s\}
19. Rxg8+ \{+M3/56 64s\} Q@f8 \{-66.88/2 12s\}
20. Rxf8\# \{+M1/127 0.012s, White mates\} 1-0


==> pgn/CrazyAraFish041_SF10/7_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "4"]
[White "CrazyAraFish-Dev-0.4.1-Rise"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "0-1"]
[PlyCount "54"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}

\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAraFish-0.4.1} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{0-1}  TimeControl 40/1800 PlyCount 54

1. e3 \{book\} d5 \{book\} 2. d4 \{book\} Bf5 \{book\} 3. Bd3 \{-0.29/24 37s\}
Bxd3 \{-0.18/26 63s\} 4. cxd3 \{+0.16/22 37s\} e6 \{0.00/29 32s\}
5. Nf3 \{+0.08/22 37s\} Nf6 \{+0.35/27 90s\} 6. Nc3 \{+0.10/26 37s\}
B@g4 \{+0.42/28 138s\} 7. B@e2 \{+0.32/25 45s\} Bd6 \{+0.68/25 15s\}
8. Ne5 \{+0.30/25 46s\} Bxe2 \{0.00/28 70s\} 9. Qxe2 \{+0.20/23 46s\}
B@h5 \{+0.35/28 86s\} 10. f3 \{-0.02/28 47s\} Nfd7 \{0.00/29 40s\}
11. B@f4 \{+1.00/27 47s\} Bxe5 \{+1.61/25 14s\} 12. dxe5 \{+0.74/29 49s\}
Nc6 \{+2.17/23 25s\} 13. B@g5 \{+0.71/28 49s\} Qxg5 \{+2.30/26 41s\}
14. Bxg5 \{+0.06/25 49s\} Ndxe5 \{+1.41/27 73s\} 15. Nxd5 \{-0.25/22 48s\}
exd5 \{+1.62/24 14s\} 16. P@f6 \{-0.82/29 49s\} g6 \{+10.34/23 38s\}
17. O-O \{-1.61/21 48s\} B@a6 \{+11.53/21 13s\} 18. e4 \{-3.59/25 47s\}
Bxd3 \{+20.98/22 24s\} 19. exd5 \{-5.91/24 47s\} Bxe2 \{+38.34/21 18s\}
20. P@d7+ \{-7.21/24 46s\} Kd8 \{+53.10/20 16s\} 21. Bce3 \{-9.20/24 44s\}
Bxf1 \{+M31/21 18s\} 22. Rxf1 \{-11.99/22 46s\} N@e2+ \{+M11/39 16s\}
23. Kf2 \{-15.96/22 33s\} N@e4+ \{+M9/45 21s\} 24. Ke1 \{-16.12/16 32s\}
R@d1+ \{+M7/50 22s\} 25. Kxd1 \{-20.66/15 16s\} P@c2+ \{+M5/50 291s\}
26. Kxe2 \{-22.20/9 15s\} P@d3+ \{+M3/101 59s\} 27. Ke1 \{-63.69/1 0.014s\}
Q@e2\# \{+M1/127 0.006s, Black mates\} 0-1


==> pgn/CrazyAraFish041_SF10/8_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "4"]
[White "stockfish-x86_64-modern  2018-11-29"]
[Black "CrazyAraFish-Dev-0.4.1-Rise"]
[Result "1-0"]
[PlyCount "55"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{Stockfish 10 x86\_64-modern  2018-11-29}
 Black: \textit{CrazyAraFish-0.4.1} Result: \textit{1-0}  TimeControl 40/1800 PlyCount 55
 
1. e3 \{book\} d5 \{book\} 2. d4 \{book\} Bf5 \{book\} 3. Bd3 \{+0.50/30 114s\}
e6 \{+0.36/23 37s\} 4. Bxf5 \{+1.00/26 14s\} exf5 \{+0.42/22 37s\}
5. Ne2 \{+0.81/27 29s\} Nf6 \{+0.35/20 37s\} 6. Nbc3 \{+1.10/27 33s\}
Nc6 \{+0.35/19 37s\} 7. Ng3 \{+1.06/25 28s\} Qd7 \{+0.33/19 44s\}
8. Bd2 \{+0.51/27 119s\} Be7 \{+0.25/18 45s\} 9. O-O \{+0.79/24 21s\}
h5 \{+1.21/22 46s\} 10. B@h4 \{+0.08/28 259s\} Ng4 \{+1.83/30 49s\}
11. Bxe7 \{-0.43/25 47s\} Nxe7 \{+1.75/28 48s\} 12. B@f4 \{-1.39/26 199s\}
h4 \{+4.01/28 48s\} 13. Nxf5 \{+1.42/22 9.9s\} Qxf5 \{+4.80/27 48s\}
14. P@h3 \{+1.67/23 21s\} Nxh2 \{+4.67/25 48s\} 15. Bxh2 \{-0.54/23 37s\}
B@h5 \{+1.46/33 49s\} 16. Bxc7 \{+4.53/21 20s\} Bxd1 \{-0.22/31 49s\}
17. N@d6+ \{0.00/25 34s\} Kf8 \{-0.11/39 49s\} 18. Nxf5 \{-2.41/26 48s\}
Nxf5 \{-0.12/28 49s\} 19. Raxd1 \{+6.55/20 17s\} B@g4 \{+0.06/26 49s\}
20. P@d7 \{+19.28/21 16s\} Bxh3 \{+1.80/30 49s\} 21. Q@e8+ \{+M15/38 8.7s\}
Rxe8 \{+5.15/1 0.014s\} 22. dxe8=R+ \{+M13/49 14s\} Kxe8 \{-M1/1 0.001s\}
23. R@d8+ \{+M11/43 17s\} Ke7 \{+3.74/1 0.016s\} 24. Nxd5+ \{+M9/57 28s\}
Ke6 \{-15.28/1 0.017s\} 25. B@d7+ \{+M7/57 66s\} Kxd5 \{-12.36/1 0.025s\}
26. P@e4+ \{+M5/58 52s\} Kxe4 \{-18.61/14 18s\} 27. Bc6+ \{+M3/58 192s\}
Q@d5 \{-71.47/2 12s\} 28. Bxd5\# \{+M1/127 0.011s, White mates\} 1-0


==> pgn/CrazyAraFish041_SF10/9_cafish_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.4.1-vs-SF10"]
[Site "?"]
[Date "2019.05.30"]
[Round "5"]
[White "CrazyAraFish-Dev-0.4.1-Rise"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "1-0"]
[PlyCount "199"]
[TimeControl "40/1800"]
[Variant "crazyhouse"]
\end{comment}

\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAraFish-0.4.1} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{1-0}  TimeControl 40/1800 PlyCount 199

1. g3 \{book\} d5 \{book\} 2. d4 \{book\} Nf6 \{book\} 3. Bg2 \{book\} Bf5 \{+0.65/29 68s\}
4. Nf3 \{+0.14/29 38s\} e6 \{+0.80/27 49s\} 5. Nc3 \{+0.30/29 38s\}
Be7 \{+0.97/29 134s\} 6. Nh4 \{+0.17/29 38s\} Bg4 \{+1.12/28 38s\}
7. O-O \{+0.58/28 38s\} Nc6 \{+1.34/29 52s\} 8. h3 \{+0.44/26 46s\} Bh5 \{+1.01/28 37s\}
9. Bg5 \{+0.22/23 45s\} O-O \{+1.12/24 33s\} 10. Qd2 \{+0.38/21 45s\}
Re8 \{+0.15/28 251s\} 11. Rad1 \{+1.58/20 44s\} a6 \{+0.62/26 71s\}
12. a3 \{+1.64/18 44s\} Rb8 \{0.00/30 81s\} 13. Qf4 \{+1.68/21 44s\} Rf8 \{0.00/26 63s\}
14. Rd3 \{+2.35/21 45s\} Ne8 \{+0.11/23 17s\} 15. Bxe7 \{+2.76/30 49s\}
Qxe7 \{+0.77/23 7.1s\} 16. B@h6 \{+2.91/26 47s\} B@f6 \{-1.67/25 197s\}
17. Bxg7 \{+3.96/24 48s\} Nxg7 \{+0.04/24 28s\} 18. P@h6 \{+4.59/23 48s\}
B@d6 \{+1.18/26 81s\} 19. Qe3 \{+4.28/28 50s\} Ne8 \{-0.93/24 30s\}
20. Nf5 \{+4.27/24 49s\} exf5 \{-1.67/25 144s\} 21. Nxd5 \{+5.89/23 49s\}
N@c4 \{-0.52/21 10s\} 22. P@g7 \{+4.05/26 51s\} Nxg7 \{+1.38/21 6.1s\}
23. Nxe7+ \{+3.84/25 52s\} Bdxe7 \{+1.38/27 47s\} 24. Qxe7 \{+3.96/32 52s\}
Nxe7 \{0.00/28 51s\} 25. B@h4 \{+4.26/26 52s\} Q@e6 \{-1.74/25 72s\}
26. hxg7 \{+3.72/29 52s\} Bxg7 \{-0.92/23 4.8s\} 27. Q@g5 \{+4.01/26 52s\}
P@f6 \{-2.49/23 24s\} 28. Qxh5 \{+4.15/27 51s\} N@d2 \{-2.36/24 23s\}
29. N@f4 \{+3.12/30 52s\} Nxf1 \{+2.26/21 5.2s\} 30. Bxf1 \{+3.12/32 52s\}
R@h6 \{0.00/24 23s\} 31. Nxe6 \{+2.63/30 52s\} fxe6 \{-1.05/25 23s\}
32. Qxh6 \{+3.48/28 52s\} Bxh6 \{-0.19/24 5.0s\} 33. B@f4 \{+2.59/26 52s\}
N@d2 \{-1.62/24 17s\} 34. Q@g2 \{+3.78/26 52s\} P@g5 \{-0.83/22 12s\}
35. Rxd2 \{+5.08/21 53s\} gxf4 \{-1.77/19 16s\} 36. gxf4+ \{+4.95/22 53s\}
Q@g6 \{-0.95/20 5.0s\} 37. R@g3 \{+3.56/32 53s\} Bxf4 \{0.00/21 14s\}
38. Rxg6+ \{+2.67/30 39s\} hxg6 \{0.00/22 10s\} 39. P@g7 \{+2.84/24 40s\}
P@h2+ \{+2.55/19 7.8s\} 40. Qxh2 \{+2.82/26 40s\} Bxh2+ \{+2.56/23 43s\}
41. Kxh2 \{+2.52/29 46s\} B@f4+ \{-6.26/26 329s\} 42. B@g3 \{+4.49/24 46s\}
Bxg3+ \{-6.44/24 45s\} 43. Bxg3 \{+4.20/24 46s\} R@h7 \{-6.41/27 113s\}
44. Rd3 \{+4.58/20 46s\} Kxg7 \{+2.34/22 56s\} 45. P@e5 \{+4.29/25 46s\}
B@e4 \{+0.74/24 163s\} 46. exf6+ \{+4.11/22 46s\} Rxf6 \{-2.52/23 69s\}
47. Q@g1 \{+4.58/26 46s\} f4 \{-1.44/24 43s\} 48. P@h6+ \{+4.24/24 46s\}
Kg8 \{-2.47/24 39s\} 49. N@g4 \{+5.03/25 46s\} fxg3+ \{-4.38/24 52s\}
50. Rxg3 \{+4.96/25 46s\} B@h4 \{-3.76/24 32s\} 51. Nxf6+ \{+4.82/24 46s\}
Bxf6 \{-3.57/23 21s\} 52. N@d7 \{+5.06/19 46s\} Bh4 \{-2.50/21 22s\}
53. R@f4 \{+6.67/25 46s\} Bxg3+ \{-3.45/25 131s\} 54. fxg3 \{+6.65/24 46s\}
Q@g5 \{-3.62/25 55s\} 55. Nf6+ \{+6.65/27 46s\} Qxf6 \{-4.73/26 42s\}
56. Rxf6 \{+6.09/29 46s\} P@f7 \{-4.45/23 15s\} 57. P@f3 \{+8.28/14 46s\}
N@h5 \{-1.43/19 46s\} 58. B@g5 \{+8.42/16 46s\} Bc6 \{-1.38/24 163s\}
59. B@g4 \{+13.37/14 46s\} Nxf6 \{-12.59/20 59s\} 60. Bxf6 \{+13.01/17 46s\}
N@d7 \{-14.78/23 100s\} 61. Bxe7 \{+18.44/18 46s\} Nd2 \{-20.19/22 70s\}
62. Bg5 \{+19.70/15 46s\} Nxf1+ \{-15.59/16 3.4s\} 63. Qxf1 \{+14.88/21 46s\}
R@e8 \{-19.52/20 20s\} 64. N@e5 \{+20.10/19 46s\} B@h8 \{-15.88/20 22s\}
65. Nxg6 \{+19.04/21 46s\} fxg6 \{-17.59/19 5.5s\} 66. P@g7 \{+17.49/20 46s\}
Bxg7 \{-20.61/21 24s\} 67. hxg7 \{+17.26/18 46s\} N@f7 \{-19.44/19 6.0s\}
68. B@e5 \{+19.10/15 46s\} P@f6 \{-23.58/17 14s\} 69. Bgxf6 \{+19.05/16 46s\}
Nxf6 \{-31.31/16 17s\} 70. Bxf6 \{+19.06/19 46s\} R@e7 \{-32.99/17 10s\}
71. Bxe7 \{+24.70/18 46s\} Rxg7 \{-35.16/16 3.3s\} 72. N@f6+ \{+23.01/19 46s\}
Kh8 \{-35.16/1 0s\} 73. Nxe8 \{+23.49/17 46s\} Rxe8 \{-32.78/15 1.8s\}
74. P@f6 \{+22.92/20 46s\} B@h6 \{-M20/16 4.5s\} 75. fxg7+ \{+21.06/20 46s\}
Bxg7 \{-M18/21 0.63s\} 76. R@h7+ \{+19.98/19 46s\} Kxh7 \{-M20/19 0.50s\}
77. N@g5+ \{+22.31/17 46s\} Nxg5 \{-28.82/12 0.44s\} 78. Bxg5 \{+23.95/20 35s\}
R@f7 \{-37.60/13 2.4s\} 79. R@h5+ \{+26.21/14 35s\} P@h6 \{-54.40/13 1.3s\}
80. Bxh6 \{+30.15/19 35s\} Bxd4 \{-42.13/8 0.72s\} 81. Bf8+ \{+25.53/20 46s\}
N@h6 \{-M12/43 132s\} 82. Rxh6+ \{+27.39/21 46s\} Kg8 \{-33.60/1 0.001s\}
83. Rxg6+ \{+29.93/18 46s\} P@g7 \{-M10/47 69s\} 84. P@h7+ \{+32.84/16 45s\}
Kxf8 \{-M8/51 44s\} 85. h8=Q+ \{+28.44/15 46s\} N@g8 \{-M12/34 34s\}
86. Rxe6 \{+28.48/16 46s\} Bg1+ \{-M10/39 100s\} 87. Qxg1 \{+33.79/16 46s\}
B@g6 \{-M8/50 32s\} 88. Rxg6 \{+34.11/15 46s\} Rxe2+ \{-M10/43 26s\}
89. P@f2 \{+38.17/13 39s\} P@h7 \{-M8/55 32s\} 90. Q@d8+ \{+33.26/16 46s\}
Be8 \{-M6/73 59s\} 91. Qxg7+ \{+31.16/18 45s\} Rxg7 \{-42.86/1 0s\}
92. R@f6+ \{+31.93/19 46s\} Nxf6 \{-M8/57 51s\} 93. Qxf6+ \{+32.51/18 46s\}
R@f7 \{-M6/64 29s\} 94. B@h6 \{+40.09/17 46s\} Rxf2+ \{-M10/45 26s\}
95. Qxf2 \{+48.91/11 23s\} Rxf6 \{-M8/66 27s\} 96. Bxg7+ \{+39.76/18 44s\}
Ke7 \{-M6/92 31s\} 97. Bxf6+ \{+48.15/16 45s\} Kd6 \{-M4/125 34s\}
98. Qd4+ \{+46.41/12 43s\} Q@d5 \{-M4/127 3.8s\} 99. R@e6+ \{+69.81/10 35s\}
Kd7 \{-M2/1 0s\} 100. R@d8\# \{+M1/1 12s, White mates\} 1-0


==> pgn/CrazyAraFish060_SF10/1_cafish060_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.6.0-vs-SF10"]
[Site "?"]
[Date "2019.07.26"]
[Round "1"]
[White "CrazyAraFish-0.6.0"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "0-1"]
[PlyCount "58"]
[TimeControl "1800+30"]
[Variant "crazyhouse"]
\end{comment}
\begin{figure}
\subsection{Matches between \alg{CrazyAraFish~0.6.0} and
%\alg{multivariant
\alg{Stockfish~10}}
\vspace{\floatsep}
\vspace{\floatsep}
\begin{minipage}{\textwidth}
\centering
\subcaptionbox{Evaluation progression for both engines\label{fig:eval_game1}}{
\includegraphics[width=\textwidth]{pgn/CrazyAraFish060_SF10/eval_plots/game1.pdf}
}
\end{minipage}
\begin{minipage}{\textwidth}
\vspace{\floatsep}
\crule
\begin{csmall}
[Event "CrazyAraFish-0.6.0-vs-SF10"]\newline
[Site "Darmstadt, GER"]\newline
[Date "2019.07.26"]\newline
[Round "1"]\newline
[White "CrazyAraFish-0.6.0"]\newline
[Black "stockfish-x86\_64-modern  2018-11-29"]\newline
[Result "0-1"]\newline
[PlyCount "58"]\newline
[TimeControl "1800+30"]\newline
[Variant "crazyhouse"]\newline
%White: \textit{CrazyAraFish-0.6.0} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{0-1}  TimeControl 1800+30 PlyCount 58

1. e4 \{book\} e5 \{book\} 2. Nf3 \{book\} Nc6 \{book\} 3. Bb5 \{book\}
Nf6 \{-0.53/29 141s\} 4. Nc3 \{+1.40/45 59s\} Be7 \{0.00/27 48s\}
5. Nxe5 \{+1.51/33 60s\} Nxe5 \{-0.92/27 83s\} 6. d4 \{+1.30/43 60s\}
Ng6 \{-1.00/29 187s\} 7. e5 \{+1.29/56 60s\} a6 \{-0.53/25 59s\}
8. P@h6 \{+2.68/52 61s\} gxh6 \{0.00/23 32s\} 9. exf6 \{+1.26/40 91s\}
Bxf6 \{0.00/26 100s\} 10. Qe2+ \{+1.14/48 60s\} N@e6 \{0.00/28 53s\}
11. Bd3 \{+2.02/36 60s\} d5 \{+0.31/24 21s\} 12. N@h5 \{+1.35/50 90s\}
Bxd4 \{+2.27/22 26s\} 13. Bxh6 \{+1.15/50 60s\} P@e4 \{+2.16/24 64s\}
14. P@g7 \{+0.63/42 60s\} Rg8 \{+2.16/24 49s\} 15. Nxe4 \{+0.27/48 60s\}
P@h3 \{+6.04/26 118s\} 16. P@f5 \{+0.04/53 61s\} hxg2 \{+9.16/22 26s\}
17. Rg1 \{+0.39/51 61s\} dxe4 \{+9.75/24 57s\} 18. fxg6 \{+0.59/49 61s\}
N@f3+ \{+14.20/23 58s\} 19. Qxf3 \{+1.07/43 62s\} exf3 \{+18.23/23 89s\}
20. gxh7 \{-1.27/51 92s\} Q@f1+ \{+M21/34 28s\} 21. Bxf1 \{-10.33/18 91s\}
P@d2+ \{+M19/39 28s\} 22. Bxd2 \{-11.66/16 60s\} Bxf2+ \{+M17/42 35s\}
23. Kxf2 \{-13.00/14 60s\} Qxd2+ \{+M15/43 50s\} 24. B@e2 \{-13.64/12 61s\}
B@d4+ \{+M13/44 34s\} 25. Kg3 \{-16.00/10 61s\} P@h4+ \{+M9/53 29s\}
26. Kxf3 \{-18.09/8 61s\} Qe3+ \{+M7/52 76s\} 27. Kg4 \{-22.57/6 62s\}
f5+ \{+M5/52 189s\} 28. Kxf5 \{-29.28/4 62s\} Nxg7+ \{+M3/61 425s\}
29. Kg6 \{-M1/2 0.028s\} Bf5\# \{+M1/127 0.009s, Black mates\} 0-1
\end{csmall}
\crule
\end{minipage}
\caption{Game 1 / 10}
\end{figure}
\addtocounter{subfigure}{-1}

==> pgn/CrazyAraFish060_SF10/2_cafish060_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.6.0-vs-SF10"]
[Site "?"]
[Date "2019.07.26"]
[Round "1"]
[White "stockfish-x86_64-modern  2018-11-29"]
[Black "CrazyAraFish-0.6.0"]
[Result "1-0"]
[PlyCount "115"]
[TimeControl "1800+30"]
[Variant "crazyhouse"]
\end{comment}
\begin{figure}
\begin{minipage}{\textwidth}
\begin{center}
\subcaptionbox{Evaluation progression for both engines}{
\includegraphics[width=\textwidth]{pgn/CrazyAraFish060_SF10/eval_plots/game2.pdf}
}
\end{center}
\label{fig:eval_game1}
\end{minipage}
\vspace{\floatsep}
%White: \textit{Stockfish 10 x86\_64-modern  2018-11-29}
% Black: \textit{CrazyAraFish-0.6.0} Result: \textit{1-0}  TimeControl 1800+30 PlyCount 115
\begin{csmall}
\crule
[Event "CrazyAraFish-0.6.0-vs-SF10"]\newline
[Site "Darmstadt, GER"]\newline
[Date "2019.07.26"]\newline
[Round "1"]\newline
[White "stockfish-x86\_64-modern  2018-11-29"]\newline
[Black "CrazyAraFish-0.6.0"]\newline
[Result "1-0"]\newline
[PlyCount "115"]\newline
[TimeControl "1800+30"]\newline
[Variant "crazyhouse"]\newline

1. e4 \{book\} e5 \{book\} 2. Nf3 \{book\} Nc6 \{book\} 3. Bb5 \{book\} Nf6 \{-1.26/33 58s\}
4. O-O \{+1.14/29 228s\} a6 \{-0.22/48 59s\} 5. Bc4 \{+1.91/27 27s\}
Be7 \{-0.25/49 59s\} 6. Nc3 \{+2.01/29 90s\} O-O \{-0.63/62 59s\}
7. d3 \{+2.05/31 120s\} d6 \{-0.60/60 59s\} 8. Ng5 \{+0.91/28 80s\} Nd4 \{-0.47/58 59s\}
9. Be3 \{+1.08/28 69s\} Qe8 \{-0.36/56 60s\} 10. Ne2 \{+1.61/27 38s\}
Nxe2+ \{+0.08/45 60s\} 11. Qxe2 \{+3.29/23 20s\} N@f4 \{+0.15/43 61s\}
12. Bxf4 \{+1.25/31 288s\} exf4 \{+0.19/42 60s\} 13. Rae1 \{+2.05/26 26s\}
B@g4 \{+0.26/36 61s\} 14. N@f3 \{+2.03/27 46s\} Kh8 \{-0.24/30 61s\}
15. N@h4 \{+3.41/26 87s\} Bce6 \{+0.22/29 61s\} 16. Bxe6 \{+4.10/24 19s\}
fxe6 \{+0.11/36 61s\} 17. e5 \{+3.41/25 80s\} dxe5 \{-0.02/50 62s\}
18. Qxe5 \{+4.10/23 37s\} Bxf3 \{-0.09/54 62s\} 19. P@h6 \{+5.24/20 19s\}
gxh6 \{-2.57/48 94s\} 20. B@g7+ \{+9.12/24 54s\} Kxg7 \{-3.29/46 61s\}
21. Qxe6 \{+9.11/24 50s\} B@e4 \{-3.83/32 62s\} 22. Nxe4 \{+9.87/26 97s\}
Qf7 \{-4.07/37 62s\} 23. Nxf6 \{+10.93/25 51s\} Bxf6 \{-4.31/34 63s\}
24. Nxf3 \{+10.99/27 117s\} Kh8 \{-4.97/31 63s\} 25. P@e7 \{+11.22/26 31s\}
Qxe6 \{-1.64/44 64s\} 26. exf8=R+ \{+6.04/25 383s\} Rxf8 \{-1.38/37 63s\}
27. Rxe6 \{+6.87/25 17s\} Q@g8 \{-1.92/40 64s\} 28. Rxf6 \{+10.16/24 57s\}
Rxf6 \{-2.97/52 96s\} 29. R@d8 \{+10.44/23 15s\} B@f8 \{-0.83/29 63s\}
30. Q@e7 \{+10.70/22 18s\} N@h3+ \{+0.53/50 64s\} 31. Kh1 \{+10.70/1 0.001s\}
R@g7 \{+0.30/21 64s\} 32. Qxf6 \{+6.25/25 72s\} P@e2 \{+0.22/19 64s\}
33. Qxg7+ \{+7.43/24 43s\} Qxg7 \{+0.15/17 65s\} 34. Rxf8+ \{+6.04/24 108s\}
Qxf8 \{+0.12/15 65s\} 35. B@d4+ \{+7.03/23 26s\} P@f6 \{+0.11/13 66s\}
36. Rg1 \{+8.26/25 25s\} Q@g7 \{+0.96/32 67s\} 37. B@h4 \{+9.33/24 23s\}
R@f1 \{+0.57/38 67s\} 38. R@a8 \{+8.07/26 202s\} Rxg1+ \{-1.29/46 102s\}
39. Nxg1 \{+8.07/1 0.001s\} Qxg2+ \{-2.00/32 66s\} 40. Kxg2 \{+8.11/1 0.001s\}
R@g7+ \{-2.83/36 67s\} 41. R@g3 \{+18.04/21 27s\} Rxg3+ \{-5.17/44 67s\}
42. fxg3 \{+19.81/23 31s\} e1=N+ \{-4.93/25 42s\} 43. Kxh3 \{+20.60/21 20s\}
P@g4+ \{-5.04/32 42s\} 44. Kxg4 \{+11.08/1 0.001s\} N@e3+ \{-4.86/34 41s\}
45. Bxe3 \{+20.28/20 20s\} R@g7+ \{-4.87/36 41s\} 46. P@g6 \{+21.33/21 66s\}
h5+ \{-5.07/39 40s\} 47. Kxf4 \{+21.24/22 120s\} Qxa8 \{-5.37/45 40s\}
48. Bc5 \{+23.08/19 27s\} R@f1+ \{-5.88/22 39s\} 49. Ke3 \{+32.99/19 27s\}
P@f2 \{-6.80/29 39s\} 50. N@f7+ \{+M17/30 14s\} Rxf7 \{-13.97/18 57s\}
51. g7+ \{+M15/35 20s\} Rxg7 \{-15.49/16 37s\} 52. N@g6+ \{+M13/45 21s\}
hxg6 \{-17.69/14 37s\} 53. Q@h6+ \{+M11/50 21s\} N@h7 \{-19.89/12 36s\}
54. Qxg7+ \{+M9/63 25s\} Kxg7 \{-21.18/10 0.048s\} 55. R@f7+ \{+M7/67 25s\}
Kxf7 \{-23.45/6 37s\} 56. R@e7+ \{+M5/73 27s\} Kg8 \{-28.76/4 37s\}
57. N@h6+ \{+M3/121 20s\} Kh8 \{-M1/2 18s\} 58. P@g7\# \{+M1/127 0.030s, White mates\}
1-0
\end{csmall}
\crule
\caption{Game 2 / 10}
\end{figure}
\addtocounter{subfigure}{-1}

==> pgn/CrazyAraFish060_SF10/3_cafish060_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.6.0-vs-SF10"]
[Site "?"]
[Date "2019.07.26"]
[Round "2"]
[White "CrazyAraFish-0.6.0"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "0-1"]
[PlyCount "74"]
[TimeControl "1800+30"]
[Variant "crazyhouse"]
\end{comment}
\begin{figure}
\begin{minipage}{\textwidth}
\centering
\subcaptionbox{Evaluation progression for both engines}{
\includegraphics[width=\textwidth]{pgn/CrazyAraFish060_SF10/eval_plots/game3.pdf}
}
\label{fig:eval_game1}
\end{minipage}
\vspace{\floatsep}
\begin{minipage}{\textwidth}
\begin{csmall}
\crule
[Event "CrazyAraFish-0.6.0-vs-SF10"]\newline
[Site "Darmstadt, GER"]\newline
[Date "2019.07.26"]\newline
[Round "2"]\newline
[White "CrazyAraFish-0.6.0"]\newline
[Black "stockfish-x86\_64-modern  2018-11-29"]\newline
[Result "0-1"]\newline
[PlyCount "74"]\newline
[TimeControl "1800+30"]\newline
[Variant "crazyhouse"]\newline

%White: \textit{CrazyAraFish-0.6.0} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{0-1}  TimeControl 1800+30 PlyCount 74
1. e4 \{book\} e5 \{book\} 2. Nf3 \{book\} Nc6 \{book\} 3. Bc4 \{book\} Bc5 \{book\}
4. O-O \{book\} Nf6 \{book\} 5. d3 \{book\} O-O \{book\} 6. Bg5 \{book\} Be7 \{book\}
7. Nbd2 \{-0.05/21 62s\} d6 \{+0.59/30 128s\} 8. Nh4 \{+0.45/40 62s\}
Na5 \{0.00/31 153s\} 9. Bxf7+ \{+1.42/65 63s\} Rxf7 \{+1.60/24 18s\}
10. P@g6 \{+1.54/63 62s\} hxg6 \{+1.77/28 79s\} 11. Nxg6 \{+1.44/42 63s\}
B@g4 \{+1.59/27 65s\} 12. Nxe7+ \{+1.59/57 63s\} Qxe7 \{+2.42/27 43s\}
13. B@f3 \{+1.66/59 63s\} Bxf3 \{+3.56/29 171s\} 14. Nxf3 \{+1.03/48 64s\}
B@h5 \{+3.90/25 16s\} 15. B@d5 \{-0.03/53 95s\} P@e6 \{+5.63/26 71s\}
16. P@h7+ \{-0.99/56 95s\} Kxh7 \{+10.27/23 17s\} 17. d4 \{-4.07/32 94s\}
Bxf3 \{+12.73/25 56s\} 18. Qxf3 \{-6.29/32 93s\} P@g4 \{+14.48/22 24s\}
19. Qe3 \{-7.28/28 61s\} exd4 \{+17.87/24 60s\} 20. Bxf6 \{-6.22/34 62s\}
gxf6 \{+18.66/23 39s\} 21. B@f5+ \{-7.01/35 62s\} exf5 \{+24.99/23 25s\}
22. exf5 \{-8.42/28 62s\} dxe3 \{+27.95/24 36s\} 23. P@g6+ \{-9.71/28 62s\}
Kg7 \{+29.84/24 52s\} 24. gxf7 \{-10.35/32 62s\} N@h3+ \{+30.87/23 35s\}
25. gxh3 \{-11.81/34 32s\} N@e2+ \{+32.14/22 48s\} 26. Kh1 \{-12.45/33 64s\}
B@e4+ \{+32.05/23 76s\} 27. N@g2 \{-12.65/32 65s\} Bxd5 \{+35.01/24 66s\}
28. R@g8+ \{-12.83/30 65s\} Kh7 \{+35.36/24 35s\} 29. Rxg4 \{-13.12/29 66s\}
Bxf5 \{+36.37/22 41s\} 30. P@g6+ \{-13.07/29 66s\} Bxg6 \{+37.67/23 111s\}
31. Rxg6 \{-13.04/29 67s\} Kxg6 \{+38.08/22 30s\} 32. N@h4+ \{-13.05/27 67s\}
Kg7 \{+41.31/21 53s\} 33. B@h6+ \{-12.43/14 68s\} Kxh6 \{+M21/21 36s\}
34. f3 \{-15.63/19 68s\} Qe5 \{+M13/40 34s\} 35. Nxe3 \{-20.14/6 69s\}
Qxh2+ \{+M5/68 92s\} 36. Kxh2 \{-24.74/4 0.12s\} P@g3+ \{+M3/109 36s\}
37. Kh1 \{-M1/2 75s\} R@h2\# \{+M1/127 0.024s, Black mates\} 0-1
\crule
\end{csmall}
\end{minipage}
\caption{Game 3 / 10}
\end{figure}
\addtocounter{subfigure}{-1}

==> pgn/CrazyAraFish060_SF10/5_cafish060_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.6.0-vs-SF10"]
[Site "?"]
[Date "2019.07.26"]
[Round "3"]
[White "CrazyAraFish-0.6.0"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "1/2-1/2"]
[PlyCount "68"]
[TimeControl "1800+30"]
[Variant "crazyhouse"]
\end{comment}
\begin{figure}
\begin{minipage}{\textwidth}
\centering
\subcaptionbox{Evaluation progression for both engines\label{fig:eval_game1}}{
\includegraphics[width=\textwidth]{pgn/CrazyAraFish060_SF10/eval_plots/game5.pdf}
}
\end{minipage}
\vspace{\floatsep}
\begin{minipage}{\textwidth}
\begin{csmall}
\crule
[Event "CrazyAraFish-0.6.0-vs-SF10"]\newline
[Site "Darmstadt, GER"]\newline
[Date "2019.07.26"]\newline
[Round "3"]\newline
[White "CrazyAraFish-0.6.0"]\newline
[Black "stockfish-x86\_64-modern  2018-11-29"]\newline
[Result "1/2-1/2"]\newline
[PlyCount "68"]\newline
[TimeControl "1800+30"]\newline
[Variant "crazyhouse"]\newline
%White: \textit{CrazyAraFish-0.6.0} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{1/2-1/2}  TimeControl 1800+30 PlyCount 74

1. e4 \{book\} Nf6 \{book\} 2. e5 \{book\} Nc6 \{book\} 3. exf6 \{book\} exf6 \{book\}
4. d4 \{book\} d5 \{book\} 5. a3 \{+0.72/38 60s\} Bd6 \{0.00/29 127s\}
6. Nc3 \{+0.39/49 60s\} Be6 \{+0.21/26 86s\} 7. Nf3 \{+0.44/40 61s\}
O-O \{-1.09/27 102s\} 8. N@h5 \{+0.10/44 61s\} Re8 \{-1.05/26 103s\}
9. Be2 \{+0.55/41 61s\} Bf8 \{-0.93/25 33s\} 10. Be3 \{+0.73/42 61s\}
Ne7 \{-1.04/27 67s\} 11. O-O \{+0.66/22 62s\} Nf5 \{0.00/27 34s\}
12. Bf4 \{+1.28/21 62s\} P@e4 \{0.00/28 29s\} 13. Ne1 \{+1.74/41 62s\}
c6 \{0.00/29 57s\} 14. Kh1 \{+1.92/46 62s\} Qb6 \{+0.37/29 92s\}
15. Bg4 \{+1.61/57 62s\} Nxd4 \{0.00/30 252s\} 16. Be3 \{+1.34/55 63s\}
Bxg4 \{+0.88/24 17s\} 17. Qxg4 \{+1.52/43 63s\} P@g6 \{0.00/30 73s\}
18. Nxg7 \{+2.01/45 64s\} Bxg7 \{0.00/32 38s\} 19. P@d7 \{+2.01/37 63s\}
Red8 \{0.00/32 82s\} 20. Nxe4 \{+1.99/47 64s\} dxe4 \{0.00/26 26s\}
21. P@e7 \{+1.27/43 64s\} B@f5 \{0.00/31 35s\} 22. exd8=R+ \{+0.71/41 65s\}
Qxd8 \{0.00/32 34s\} 23. R@e8+ \{+0.42/39 65s\} Qxe8 \{0.00/33 35s\}
24. dxe8=R+ \{+0.12/62 65s\} Rxe8 \{0.00/33 59s\} 25. Bxd4 \{+0.04/16 66s\}
Bxg4 \{0.00/33 79s\} 26. Bxf6 \{+0.05/14 66s\} Q@h5 \{0.00/32 69s\}
27. Bxg7 \{+0.06/12 66s\} N@g3+ \{0.00/34 80s\} 28. fxg3 \{+0.01/10 66s\}
R@g1+ \{0.00/35 100s\} 29. Kxg1 \{0.00/8 67s\} N@e2+ \{0.00/33 138s\}
30. Kh1 \{0.00/6 67s\} Nxg3+ \{0.00/35 375s\} 31. Kg1 \{0.00/4 0.005s\}
Ne2+ \{0.00/36 25s\} 32. Kh1 \{0.00/2 72s\} Ng3+ \{0.00/38 221s\}
33. Kg1 \{0.00/1 0.006s\} Ne2+ \{0.00/36 125s\} 34. Kh1 \{0.00/1 77s\}
Ng3+ \{0.00/40 22s, Draw by 3-fold repetition\} 1/2-1/2
\end{csmall}
\crule
\end{minipage}
\caption{Game 5 / 10}
\end{figure}
\addtocounter{subfigure}{-1}

==> pgn/CrazyAraFish060_SF10/6_cafish060_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.6.0-vs-SF10"]
[Site "?"]
[Date "2019.07.26"]
[Round "3"]
[White "stockfish-x86_64-modern  2018-11-29"]
[Black "CrazyAraFish-0.6.0"]
[Result "1-0"]
[PlyCount "77"]
[TimeControl "1800+30"]
[Variant "crazyhouse"]
\end{comment}
\begin{figure}
\begin{minipage}{\textwidth}
\centering
\subcaptionbox{Game 6 / 10: Evaluation progression for both engines}{
\includegraphics[width=\textwidth]{pgn/CrazyAraFish060_SF10/eval_plots/game6.pdf}
}
\label{fig:eval_game1}
\end{minipage}

\begin{minipage}{\textwidth}
\vspace{\floatsep}
\begin{csmall}
\crule
[Event "CrazyAraFish-0.6.0-vs-SF10"]\newline
[Site "Darmstadt, GER"]\newline
[Date "2019.07.26"]\newline
[Round "3"]\newline
[White "stockfish-x86\_64-modern  2018-11-29"]\newline
[Black "CrazyAraFish-0.6.0"]\newline
[Result "1-0"]\newline
[PlyCount "77"]\newline
[TimeControl "1800+30"]\newline
[Variant "crazyhouse"]\newline
%White: \textit{Stockfish 10 x86\_64-modern  2018-11-29}
% Black: \textit{CrazyAraFish-0.6.0} Result: \textit{1-0}  TimeControl 1800+30 PlyCount 77
 
1. e4 \{book\} Nf6 \{book\} 2. e5 \{book\} Nc6 \{book\} 3. exf6 \{book\} exf6 \{book\}
4. d4 \{book\} d5 \{book\} 5. a3 \{+1.67/28 126s\} Be7 \{-0.26/38 60s\}
6. Nc3 \{+2.34/26 78s\} O-O \{-0.22/51 60s\} 7. Be2 \{+2.46/27 37s\}
Re8 \{-0.59/50 61s\} 8. Nf3 \{+1.71/28 124s\} Bf8 \{+0.02/45 61s\}
9. Be3 \{+1.43/30 388s\} Ne7 \{+0.33/34 61s\} 10. N@h4 \{+1.83/26 20s\}
P@e4 \{+0.82/28 61s\} 11. Nd2 \{+1.50/28 66s\} g5 \{+0.97/40 62s\}
12. Ndxe4 \{+2.87/28 45s\} dxe4 \{-0.03/46 92s\} 13. Bc4 \{+3.53/26 43s\}
N@d6 \{+4.20/40 61s\} 14. Nxe4 \{+3.78/25 34s\} Nef5 \{-2.28/36 92s\}
15. Nxf5 \{+7.35/24 26s\} Bxf5 \{-1.73/43 61s\} 16. Nxd6 \{+7.64/25 24s\}
cxd6 \{-1.62/29 61s\} 17. N@g3 \{+8.23/25 76s\} N@h4 \{-1.33/38 62s\}
18. O-O \{+8.98/25 28s\} N@h3+ \{-1.15/43 61s\} 19. gxh3 \{+10.93/25 19s\}
Bxh3 \{-1.45/47 62s\} 20. Bxf7+ \{+11.94/24 44s\} Kxf7 \{-2.04/43 62s\}
21. d5 \{+13.70/24 61s\} P@g2 \{-1.90/37 63s\} 22. Re1 \{+15.03/25 30s\}
Qa5 \{-0.73/42 63s\} 23. b4 \{+18.24/21 32s\} Qb5 \{-4.14/40 94s\}
24. P@e6+ \{+20.23/23 50s\} Rxe6 \{-6.72/38 93s\} 25. dxe6+ \{+21.29/19 33s\}
Bxe6 \{-7.37/36 61s\} 26. P@e7 \{+25.00/19 38s\} P@d2 \{-7.60/34 62s\}
27. Bxd2 \{+31.57/21 70s\} P@e2 \{-4.83/26 63s\} 28. exf8=R+ \{+41.73/22 99s\}
Kxf8 \{-6.98/32 94s\} 29. P@e7+ \{+44.38/20 25s\} Kxe7 \{-8.36/26 61s\}
30. Qxe2 \{+46.30/20 48s\} Qxe2 \{-10.05/30 62s\} 31. N@d5+ \{+M19/27 27s\}
Kf8 \{-10.99/28 62s\} 32. P@e7+ \{+M17/31 31s\} Kf7 \{-12.08/26 63s\}
33. R@f8+ \{+M15/35 44s\} Rxf8 \{-13.92/18 63s\} 34. exf8=Q+ \{+M13/44 32s\}
Kxf8 \{-15.47/16 32s\} 35. P@e7+ \{+M11/51 42s\} Kg7 \{-17.56/8 66s\}
36. e8=N+ \{+M7/61 158s\} Kf7 \{-22.48/6 67s\} 37. R@e7+ \{+M5/65 35s\}
Kg6 \{-31.00/4 67s\} 38. N@f8+ \{+M3/71 74s\} Kh6 \{-M1/2 0.040s\}
39. Rxh7\# \{+M1/127 0.010s, White mates\} 1-0
\crule
\end{csmall}
\end{minipage}
\caption{Game 6 / 10}
\end{figure}
\addtocounter{subfigure}{-1}

==> pgn/CrazyAraFish060_SF10/7_cafish060_sf10.tex <==
\begin{comment}
[Event "CrazyAraFish-0.6.0-vs-SF10"]
[Site "?"]
[Date "2019.07.26"]
[Round "1"]
[White "CrazyAraFish-0.6.0"]
[Black "stockfish-x86_64-modern  2018-11-29"]
[Result "0-1"]
[PlyCount "112"]
[TimeControl "1800+30"]
[Variant "crazyhouse"]
\end{comment}
\begin{figure}
\begin{minipage}{\textwidth}
\centering
\subcaptionbox{Evaluation progression for both engines\label{fig:eval_game1}}{
\includegraphics[width=\textwidth]{pgn/CrazyAraFish060_SF10/eval_plots/game7.pdf}
}
\end{minipage}
%White: \textit{CrazyAraFish-0.6.0} Black: \textit{Stockfish 10 x86\_64-modern  2018-11-29} Result: \textit{0-1}  TimeControl 1800+30 PlyCount 112
\vspace{\floatsep}
\begin{minipage}{\textwidth}
\crule
\begin{csmall}
[Event "CrazyAraFish-0.6.0-vs-SF10"]\newline
[Site "Darmstadt, GER"]\newline
[Date "2019.07.26"]\newline
[Round "4"]\newline
[White "CrazyAraFish-0.6.0"]\newline
[Black "stockfish-x86\_64-modern  2018-11-29"]\newline
[Result "0-1"]\newline
[PlyCount "112"]\newline
[TimeControl "1800+30"]\newline
[Variant "crazyhouse"]\newline

1. e3 \{book\} d5 \{book\} 2. d4 \{book\} Bf5 \{book\} 3. Bd3 \{-0.22/23 58s\}
e6 \{+0.16/31 175s\} 4. Nc3 \{-0.23/23 59s\} Bxd3 \{+0.35/31 130s\}
5. cxd3 \{+0.06/31 30s\} Nf6 \{+0.35/26 17s\} 6. Nf3 \{+0.22/25 60s\}
B@g4 \{+0.19/27 125s\} 7. B@e2 \{+0.02/31 60s\} Bd6 \{+0.63/25 15s\}
8. Ne5 \{+0.17/42 60s\} Bxe2 \{+0.75/27 54s\} 9. Nxe2 \{+0.02/37 60s\}
Nc6 \{+2.82/27 47s\} 10. B@g3 \{0.00/34 61s\} Bxe5 \{+2.82/26 32s\}
11. dxe5 \{0.00/28 61s\} Ng4 \{+3.27/26 78s\} 12. Nd4 \{-0.77/34 92s\}
Ngxe5 \{+4.21/24 29s\} 13. Nxc6 \{-1.18/34 61s\} Nxc6 \{+4.55/27 96s\}
14. O-O \{-1.84/28 61s\} O-O \{+5.03/25 54s\} 15. N@h5 \{-0.04/37 61s\}
B@e4 \{+4.27/26 287s\} 16. f3 \{-1.06/40 92s\} Bxf3 \{+4.28/27 152s\}
17. Qxf3 \{-0.21/32 61s\} N@g5 \{+5.43/27 23s\} 18. Qe2 \{-0.42/41 61s\}
P@e4 \{+5.64/24 16s\} 19. B@f6 \{-0.76/44 61s\} P@f3 \{+5.04/26 74s\}
20. gxf3 \{-0.89/44 61s\} exf3 \{+5.43/30 132s\} 21. Rxf3 \{-0.41/52 62s\}
N@h3+ \{+5.61/29 148s\} 22. Kh1 \{-0.14/37 62s\} Nxf3 \{+4.84/28 76s\}
23. Bd2 \{-0.92/38 94s\} Nxd2 \{+5.24/26 54s\} 24. B@g4 \{-1.17/37 61s\}
gxf6 \{+5.99/25 31s\} 25. P@g7 \{-1.30/35 62s\} B@h6 \{+6.13/25 18s\}
26. gxf8=Q+ \{-0.72/37 63s\} Bxf8 \{+6.60/26 79s\} 27. R@e8 \{-1.32/19 63s\}
Qxe8 \{+3.94/26 163s\} 28. Nxf6+ \{+0.76/20 63s\} Kh8 \{+5.11/24 29s\}
29. Nxe8 \{+0.50/40 63s\} R@g6 \{+5.12/25 30s\} 30. Q@c3+ \{-0.01/43 96s\}
B@e5 \{+5.62/26 64s\} 31. Qcxd2 \{-0.20/28 63s\} Rxe8 \{+5.74/25 75s\}
32. N@h4 \{+0.25/44 63s\} N@f2+ \{+6.69/23 21s\} 33. Bxf2 \{-0.94/37 95s\}
Nxf2+ \{+7.89/25 47s\} 34. Qxf2 \{-1.14/35 31s\} Rxg4 \{+8.15/24 26s\}
35. P@g7+ \{-1.17/40 65s\} Bexg7 \{+10.48/25 108s\} 36. P@g6 \{-0.65/44 66s\}
hxg6 \{+14.48/22 25s\} 37. Qxf7 \{-4.83/30 99s\} Rxh4 \{+21.37/22 18s\}
38. Qff2 \{-6.27/22 96s\} B@f3+ \{+25.59/24 37s\} 39. Qxf3 \{-7.54/28 62s\}
Ne5 \{+25.80/22 13s\} 40. B@f6 \{-7.79/27 63s\} Nxf3 \{+36.99/25 28s\}
41. N@f7+ \{-8.05/30 43s\} Kg8 \{+39.41/25 47s\} 42. Bxh4 \{-8.19/33 42s\}
P@h3 \{+41.51/23 62s\} 43. Nh6+ \{-9.88/25 41s\} Kh7 \{+44.90/19 23s\}
44. P@g2 \{-11.43/20 41s\} Q@h5 \{+49.26/20 65s\} 45. R@f2 \{-10.44/24 40s\}
hxg2+ \{+55.72/19 25s\} 46. Rxg2 \{-11.09/22 40s\} Nxd2 \{+M35/21 51s\}
47. N@g5+ \{-10.17/18 39s\} Kxh6 \{+M29/21 18s\} 48. Rxd2 \{-10.85/28 39s\}
Qxh4 \{+M21/25 39s\} 49. P@g3 \{-11.93/14 38s\} P@h3 \{+M17/31 32s\}
50. N@g8+ \{-14.79/14 38s\} Kh5 \{+M15/39 18s\} 51. gxh4 \{-16.80/10 37s\}
B@f3+ \{+M11/42 19s\} 52. Nxf3 \{-17.47/10 37s\} P@g2+ \{+M9/51 31s\}
53. Rxg2 \{-20.33/8 37s\} hxg2+ \{+M7/55 100s\} 54. Kxg2 \{-22.83/6 36s\}
P@h3+ \{+M5/57 75s\} 55. Kf1 \{-26.40/4 36s\} Q@g2+ \{+M3/59 32s\}
56. Ke1 \{-M1/2 0.028s\} R@f1\# \{+M1/127 0.022s, Black mates\} 0-1
\end{csmall}
\crule
\end{minipage}
\caption{Game 7 / 10}
\end{figure}
\addtocounter{subfigure}{-1}

==> pgn/JannLee/1/lichess_pgn_2018.12.21_CrazyAra_vs_JannLee.FXeJuDCa.tex <==
[Event "Rated Crazyhouse game"]
[Site "https://lichess.org/FXeJuDCa"]
[Date "2018.12.21"]
[Round "-"]
[White "CrazyAra"]
[Black "JannLee"]
[Result "1-0"]
[UTCDate "2018.12.21"]
[UTCTime "18:02:51"]
[WhiteElo "2594"]
[BlackElo "2649"]
[WhiteRatingDiff "+16"]
[BlackRatingDiff "-8"]
[WhiteTitle "BOT"]
[BlackTitle "LM"]
[Variant "Crazyhouse"]
[TimeControl "300+15"]
[ECO "?"]
[Opening "?"]
[Termination "Normal"]

1. e4 e6 2. Nc3 d5 3. exd5 exd5 4. Bb5+ c6 5. Qe2+ P@e6 6. Bd3 Nd7 7. Nf3 Nc5 8. O-O Nxd3 9. cxd3 Nf6 10. d4 Be7 11. d3 O-O 12. P@h6 gxh6 13. Bxh6 P@g7 14. Bxg7 Kxg7 15. P@g5 Kh8 16. gxf6 Bxf6 17. P@e5 Bg7 18. N@h5 B@h6 19. Nxg7 Bxg7 20. B@f6 Bxf6 21. exf6 Qxf6 22. B@e5 B@g7 23. Bxf6 Bxf6 24. N@h5 B@g7 25. Nxf6 Bxf6 26. B@e5 B@g7 27. Bxf6 Bxf6 28. B@e5 B@g7 29. Nxd5 exd5 30. Bxf6 Bxf6 31. B@e5 B@g7 32. Bxf6 Bxf6 33. B@g5 B@g7 34. P@h6 N@f5 35. hxg7+ Bxg7 36. B@f6 N@h5 37. Bxg7+ Nhxg7 38. B@f6 N@e8 39. Bxg7+ Nexg7 40. Bf6 B@h6 41. N@g4 B@f4 42. Nxh6 Bxh6 43. B@g5 N@h5 44. Bxh6 Nxf6 45. Bxg7+ Nxg7 46. B@h6 Rg8 47. Ng5 B@e6 48. N@e5 B@e8 49. Q@e7 Ngh5 50. Qxh5 Nxh5 51. Qxf7 Rxg5 52. Qxe8+ Q@g8 53. N@f7+ Bxf7 54. Nxf7# 1-0




==> pgn/JannLee/1_crazya_jannlee.tex <==
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAra 0.3.1} Black: \textit{LM JannLee} Result: \textit{1-0}  Site: \url{https://lichess.org/FXeJuDCa}

1. e4 e6 2. Nc3 d5 3. exd5 exd5 4. Bb5+ c6 5. Qe2+ P@e6 6. Bd3 Nd7 7. Nf3 Nc5 8. O-O Nxd3 9. cxd3 Nf6 10. d4 Be7 11. d3 O-O 12. P@h6 gxh6 13. Bxh6 P@g7 14. Bxg7 Kxg7 15. P@g5 Kh8 16. gxf6 Bxf6 17. P@e5 Bg7 18. N@h5 B@h6 19. Nxg7 Bxg7 20. B@f6 Bxf6 21. exf6 Qxf6 22. B@e5 B@g7 23. Bxf6 Bxf6 24. N@h5 B@g7 25. Nxf6 Bxf6 26. B@e5 B@g7 27. Bxf6 Bxf6 28. B@e5 B@g7 29. Nxd5 exd5 30. Bxf6 Bxf6 31. B@e5 B@g7 32. Bxf6 Bxf6 33. B@g5 B@g7 34. P@h6 N@f5 35. hxg7+ Bxg7 36. B@f6 N@h5 37. Bxg7+ Nhxg7 38. B@f6 N@e8 39. Bxg7+ Nexg7 40. Bf6 B@h6 41. N@g4 B@f4 42. Nxh6 Bxh6 43. B@g5 N@h5 44. Bxh6 Nxf6 45. Bxg7+ Nxg7 46. B@h6 Rg8 47. Ng5 B@e6 48. N@e5 B@e8 49. Q@e7 Ngh5 50. Qxh5 Nxh5 51. Qxf7 Rxg5 52. Qxe8+ Q@g8 53. N@f7+ Bxf7 54. Nxf7\# 1-0
%TimeControl: \textit{300+15}

==> pgn/JannLee/2/lichess_pgn_2018.12.21_JannLee_vs_CrazyAra.j9eQS4TF.tex <==
[Event "Rated Crazyhouse game"]
[Site "https://lichess.org/j9eQS4TF"]
[Date "2018.12.21"]
[Round "-"]
[White "JannLee"]
[Black "CrazyAra"]
[Result "1-0"]
[UTCDate "2018.12.21"]
[UTCTime "18:33:01"]
[WhiteElo "2641"]
[BlackElo "2610"]
[WhiteRatingDiff "+6"]
[BlackRatingDiff "-13"]
[WhiteTitle "LM"]
[BlackTitle "BOT"]
[Variant "Crazyhouse"]
[TimeControl "300+15"]
[ECO "?"]
[Opening "?"]
[Termination "Normal"]

1. e4 Nc6 2. Nc3 Nf6 3. d4 d5 4. e5 Ne4 5. Bb5 a6 6. Bxc6+ bxc6 7. Nge2 Bf5 8. O-O e6 9. f3 Nxc3 10. bxc3 h5 11. N@e3 N@h4 12. N@a5 B@d7 13. Nxf5 Nxf5 14. B@b7 N@e3 15. Nxc6 Nxd1 16. Nxd8 Rxd8 17. Rxd1 Q@b5 18. Bxa6 Qxa6 19. P@d3 N@e3 20. Bxe3 Nxe3 21. P@d6 Nxd1 22. Rxd1 B@e3+ 23. Kh1 Bxd6 24. exd6 Qxd6 25. B@b4 Qxb4 26. cxb4 P@f2 27. Q@f1 R@g1+ 28. Qxg1 fxg1=Q+ 29. Rxg1 P@f2 30. N@g6 fxg1=Q+ 31. Nxg1 Q@e7 32. Q@d6 fxg6 33. Qxe7+ Kxe7 34. R@f7+ Kxf7 35. N@e5+ Kg8 36. N@f6+ gxf6 37. Q@f7# 1-0




==> pgn/JannLee/2_jannlee_crazyara.tex <==
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{LM JannLee} Black: \textit{ CrazyAra 0.3.1} Result: \textit{1-0}  Site: \url{https://lichess.org/j9eQS4TF}

1. e4 Nc6 2. Nc3 Nf6 3. d4 d5 4. e5 Ne4 5. Bb5 a6 6. Bxc6+ bxc6 7. Nge2 Bf5 8. O-O e6 9. f3 Nxc3 10. bxc3 h5 11. N@e3 N@h4 12. N@a5 B@d7 13. Nxf5 Nxf5 14. B@b7 N@e3 15. Nxc6 Nxd1 16. Nxd8 Rxd8 17. Rxd1 Q@b5 18. Bxa6 Qxa6 19. P@d3 N@e3 20. Bxe3 Nxe3 21. P@d6 Nxd1 22. Rxd1 B@e3+ 23. Kh1 Bxd6 24. exd6 Qxd6 25. B@b4 Qxb4 26. cxb4 P@f2 27. Q@f1 R@g1+ 28. Qxg1 fxg1=Q+ 29. Rxg1 P@f2 30. N@g6 fxg1=Q+ 31. Nxg1 Q@e7 32. Q@d6 fxg6 33. Qxe7+ Kxe7 34. R@f7+ Kxf7 35. N@e5+ Kg8 36. N@f6+ gxf6 37. Q@f7\# 1-0
%TimeControl: \textit{300+15}

==> pgn/JannLee/3/lichess_pgn_2018.12.21_CrazyAra_vs_JannLee.CYUSIV9C.tex <==
[Event "Rated Crazyhouse game"]
[Site "https://lichess.org/CYUSIV9C"]
[Date "2018.12.21"]
[Round "-"]
[White "CrazyAra"]
[Black "JannLee"]
[Result "1-0"]
[UTCDate "2018.12.21"]
[UTCTime "18:56:14"]
[WhiteElo "2597"]
[BlackElo "2647"]
[WhiteRatingDiff "+16"]
[BlackRatingDiff "-8"]
[WhiteTitle "BOT"]
[BlackTitle "LM"]
[Variant "Crazyhouse"]
[TimeControl "300+15"]
[ECO "?"]
[Opening "?"]
[Termination "Normal"]

1. e4 e5 2. Nc3 Bc5 3. Nf3 d6 4. Be2 Nf6 5. O-O O-O 6. d3 c6 7. Bg5 Be6 8. d4 exd4 9. Nxd4 Bxd4 10. Qxd4 c5 11. Qxf6 gxf6 12. P@e7 Qxe7 13. N@d5 Q@d8 14. Nxe7+ Qxe7 15. B@g7 Kxg7 16. Q@h6+ Kg8 17. Bxf6 Qxf6 18. Qxf6 P@g7 19. P@h6 B@h8 20. hxg7 Bxg7 21. Qxg7+ Kxg7 22. P@h6+ Kf6 23. B@h4+ P@g5 24. Bxg5+ Kxg5 25. f4+ Kxh6 26. Q@g5# 1-0




==> pgn/JannLee/3_crazyara_jannlee.tex <==
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAra 0.3.1} Black: \textit{LM JannLee} Result: \textit{1-0}   Site: \url{https://lichess.org/CYUSIV9C}

1. e4 e5 2. Nc3 Bc5 3. Nf3 d6 4. Be2 Nf6 5. O-O O-O 6. d3 c6 7. Bg5 Be6 8. d4 exd4 9. Nxd4 Bxd4 10. Qxd4 c5 11. Qxf6 gxf6 12. P@e7 Qxe7 13. N@d5 Q@d8 14. Nxe7+ Qxe7 15. B@g7 Kxg7 16. Q@h6+ Kg8 17. Bxf6 Qxf6 18. Qxf6 P@g7 19. P@h6 B@h8 20. hxg7 Bxg7 21. Qxg7+ Kxg7 22. P@h6+ Kf6 23. B@h4+ P@g5 24. Bxg5+ Kxg5 25. f4+ Kxh6 26. Q@g5\# 1-0
%TimeControl: \textit{300+15}

==> pgn/JannLee/4/lichess_pgn_2018.12.21_JannLee_vs_CrazyAra.EeOl3trm.tex <==
[Event "Rated Crazyhouse game"]
[Site "https://lichess.org/EeOl3trm"]
[Date "2018.12.21"]
[Round "-"]
[White "JannLee"]
[Black "CrazyAra"]
[Result "0-1"]
[UTCDate "2018.12.21"]
[UTCTime "19:07:02"]
[WhiteElo "2639"]
[BlackElo "2613"]
[WhiteRatingDiff "-7"]
[BlackRatingDiff "+14"]
[WhiteTitle "LM"]
[BlackTitle "BOT"]
[Variant "Crazyhouse"]
[TimeControl "300+15"]
[ECO "?"]
[Opening "?"]
[Termination "Normal"]

1. e4 e6 2. d4 d5 3. e5 Nc6 4. Nf3 Nge7 5. Bd3 Nf5 6. Bg5 Be7 7. Bxe7 Qxe7 8. B@c5 Nh4 9. Bxe7 Nxg2+ 10. Kf1 Nxe7 11. Kxg2 P@e4 12. Bb5+ B@d7 13. Be2 exf3+ 14. Bxf3 B@e4 15. Kg1 Bxf3 16. Qxf3 B@e4 17. Qxf7+ Kxf7 18. N@h6+ Ke8 19. P@f7+ Kd8 20. Q@g8+ Q@f8 21. Qxh8 Qxh8 22. R@g8+ N@f8 23. B@f1 gxh6 0-1




==> pgn/JannLee/4_jannlee_crazyara.tex <==
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{LM JannLee} Black: \textit{ CrazyAra 0.3.1} Result: \textit{0-1}  Site: \url{https://lichess.org/EeOl3trm}

1. e4 e6 2. d4 d5 3. e5 Nc6 4. Nf3 Nge7 5. Bd3 Nf5 6. Bg5 Be7 7. Bxe7 Qxe7 8. B@c5 Nh4 9. Bxe7 Nxg2+ 10. Kf1 Nxe7 11. Kxg2 P@e4 12. Bb5+ B@d7 13. Be2 exf3+ 14. Bxf3 B@e4 15. Kg1 Bxf3 16. Qxf3 B@e4 17. Qxf7+ Kxf7 18. N@h6+ Ke8 19. P@f7+ Kd8 20. Q@g8+ Q@f8 21. Qxh8 Qxh8 22. R@g8+ N@f8 23. B@f1 gxh6 0-1
%TimeControl: \textit{300+15}

==> pgn/JannLee/5/lichess_pgn_2018.12.21_CrazyAra_vs_JannLee.v1ABi8LI.tex <==
[Event "Rated Crazyhouse game"]
[Site "https://lichess.org/v1ABi8LI"]
[Date "2018.12.21"]
[Round "-"]
[White "CrazyAra"]
[Black "JannLee"]
[Result "1-0"]
[UTCDate "2018.12.21"]
[UTCTime "19:28:57"]
[WhiteElo "2627"]
[BlackElo "2632"]
[WhiteRatingDiff "+13"]
[BlackRatingDiff "-7"]
[WhiteTitle "BOT"]
[BlackTitle "LM"]
[Variant "Crazyhouse"]
[TimeControl "300+15"]
[ECO "?"]
[Opening "?"]
[Termination "Normal"]

1. e4 Nf6 2. Nc3 d5 3. exd5 Nxd5 4. Bb5+ Nc6 5. Nf3 P@h3 6. Rg1 hxg2 7. P@a6 Nxc3 8. bxc3 N@d6 9. axb7 Bxb7 10. P@a6 Nxb5 11. axb7 Rb8 12. B@c4 Nd6 13. Bxf7+ Kxf7 14. Rxg2 B@g6 15. P@h5 Kg8 16. hxg6 hxg6 17. P@e6 B@e8 18. N@g5 Rxb7 19. B@f7+ Nxf7 20. exf7+ Bxf7 21. Nxf7 Qd5 22. Nxh8 Kxh8 23. N@f4 Qe4+ 24. B@e3 N@e5 25. Nxg6+ Qxg6 26. Rxg6 Nxg6 27. P@f7 R@h1+ 28. R@g1 Rxg1+ 29. Nxg1 N@g2+ 30. Kf1 Nxe3+ 31. dxe3 B@c4+ 32. R@d3 Bxf7 33. N@g5 B@g8 34. Nxf7+ Bxf7 35. B@e4 N@e5 36. f4 P@f5 37. Bg2 Ng4 38. Qxg4 fxg4 39. N@g5 Q@g8 40. Q@h5+ R@h6 41. Qxg4 P@b2 42. Bxb2 Rxb2 43. Nxf7+ Qxf7 44. B@e6 B@g8 45. Bxf7 Bxf7 46. P@e6 Bg8 47. P@f7 Bh7 48. Qxg6 Rxg6 49. Q@g8+ Bxg8 50. fxg8=Q+ Kxg8 51. B@f7+ Kh8 52. Bxg6 Q@f2+ 53. Kxf2 Rxc2+ 54. R@d2 B@h4+ 55. N@g3 N@g4+ 56. Kf3 Nxh2+ 57. Ke2 Rxd2+ 58. Kxd2 R@f2+ 59. R@e2 Q@b2+ 60. Q@c2 Qxa1 61. Rxf2 Qxg1 62. R@h7+ Kg8 63. Bf7+ Kxh7 64. Rd8+ 1-0




==> pgn/JannLee/5_crazyara_jannlee.tex <==
\noindent\makebox[\linewidth]{\rule{\textwidth}{0.4pt}}
White: \textit{CrazyAra 0.3.1} Black: \textit{LM JannLee} Result: \textit{1-0}   Site: \url{https://lichess.org/v1ABi8LI}

1. e4 Nf6 2. Nc3 d5 3. exd5 Nxd5 4. Bb5+ Nc6 5. Nf3 P@h3 6. Rg1 hxg2 7. P@a6 Nxc3 8. bxc3 N@d6 9. axb7 Bxb7 10. P@a6 Nxb5 11. axb7 Rb8 12. B@c4 Nd6 13. Bxf7+ Kxf7 14. Rxg2 B@g6 15. P@h5 Kg8 16. hxg6 hxg6 17. P@e6 B@e8 18. N@g5 Rxb7 19. B@f7+ Nxf7 20. exf7+ Bxf7 21. Nxf7 Qd5 22. Nxh8 Kxh8 23. N@f4 Qe4+ 24. B@e3 N@e5 25. Nxg6+ Qxg6 26. Rxg6 Nxg6 27. P@f7 R@h1+ 28. R@g1 Rxg1+ 29. Nxg1 N@g2+ 30. Kf1 Nxe3+ 31. dxe3 B@c4+ 32. R@d3 Bxf7 33. N@g5 B@g8 34. Nxf7+ Bxf7 35. B@e4 N@e5 36. f4 P@f5 37. Bg2 Ng4 38. Qxg4 fxg4 39. N@g5 Q@g8 40. Q@h5+ R@h6 41. Qxg4 P@b2 42. Bxb2 Rxb2 43. Nxf7+ Qxf7 44. B@e6 B@g8 45. Bxf7 Bxf7 46. P@e6 Bg8 47. P@f7 Bh7 48. Qxg6 Rxg6 49. Q@g8+ Bxg8 50. fxg8=Q+ Kxg8 51. B@f7+ Kh8 52. Bxg6 Q@f2+ 53. Kxf2 Rxc2+ 54. R@d2 B@h4+ 55. N@g3 N@g4+ 56. Kf3 Nxh2+ 57. Ke2 Rxd2+ 58. Kxd2 R@f2+ 59. R@e2 Q@b2+ 60. Q@c2 Qxa1 61. Rxf2 Qxg1 62. R@h7+ Kg8 63. Bf7+ Kxh7 64. Rd8+ 1-0
%TimeControl: \textit{300+15}

==> tables/strength_eval_ca041.tex <==
\begin{table}[]
\centering
\caption{\alg{CrazyAra 0.4.1's} CPU match results playing twelve different crazyhouse engines. \textbf{Wapc} and \textbf{Lapc} means ``win average ply count'' and ``loss average ply count'' from \textit{CrazyAra's} perspective describing the average game length. *PyChess' rating of \num{1566.25} corresponds to version 0.12.4, Immortal's rating of \num{2997.33} corresponds to version 3.04, \alg{Stockfish}'s rating of \num{3946.06} corresponds to version 2017-09-23 using a single thread instead of eight. Engine dentoted with \textdagger $\,$ use Wine for emulation. For more information about the engines and their corresponding authors please refer to \small{\url{http://rwbc-chess.de/chronology.htm}} \normalsize created by  Simon Guenther} %and \url{https://lichess.org/forum/team-crazyhouse-engine-development-and-game-analyses/swiss-crazyhouse-tournament?page=3}}
\label{tab:strength_eval_cpu}
\vspace{.2cm}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Engine Name} & \textbf{Version}         & \textbf{Elo Rating}             & \textbf{NPS (Million)}       & \textbf{Wapc}     & \textbf{Lapc}    & \textbf{+}  & \textbf{=} & \textbf{-}   \\
\midrule %
PyChess     & 1.1             & \textgreater{}\num{1566.25}* & \num{0.012} & $37\pm6$   & -       & \num{10} & \num{0} & \num{0}  \\ 
KKFChess \textdagger    & 2.6.7b          & \num{1849.50}                & \num{2.9}   & $56\pm16$  & -       & \num{10} & \num{0} & \num{0}  \\ 
TSCP ZH     & 1.1             & \num{1888.47}                & \num{0.5}   & $60\pm12$  & -       & \num{10} & \num{0} & \num{0}  \\ 
Pulsar      & 2009-9b         & \num{1982.07}                & ?.?    & $63\pm16$  & -       & \num{10} & \num{0} & \num{0}  \\ 
Feuerstein \textdagger  & 0.4.6.1         & \num{2205.74}                & \num{0.1}   & $53\pm13$  & -       & \num{10} & \num{0} & \num{0}  \\ 
Nebiyu \textdagger     & 1.45a           & \num{2244.39}                & \num{1.5}   & $51\pm17$  & -       & \num{10} & \num{0} & \num{0}  \\ 
SjaakII     & 1.4.1           & \num{2245.56}                & \num{0.425}  & $56\pm10$  & -       & \num{10} & \num{0} & \num{0}  \\ 
Sjeng       & 11.2            & \num{2300.00}                & \num{0.7}   & $72\pm16$  & -       & \num{10} & \num{0} & \num{0}  \\ 
CrazyWa     & 1.0.1           & \num{2500.00}                & \num{1.4}   & $82\pm20$  & -       & \num{10} & \num{0} & \num{0}  \\ 
Sunsetter   & 9               & \num{2703.39}                & \num{1.5}   & $63\pm22$  & $68\pm0$  & \num{9}  & \num{0} & \num{1}  \\ 
TjChess     & 1.37            & \num{2732.58}                & \num{1.37}  & $80\pm22$  & -       & \num{10} & \num{0} & \num{0}  \\ 
Imortal \textdagger     & 4.3             & \textgreater{}\num{2997.33}* & 0.9   & $113\pm39$ & $89\pm48$ & \num{7}  & \num{0} & \num{3}  \\ 
Stockfish   & 10 (2018-11-29) & \textgreater{}\num{3946.06}* & 4.6   & -        & $72\pm24$ & \num{0}  & \num{0} & \num{10} \\
\bottomrule
\end{tabular}
\end{table}
